Leveraging Causal Graphs for Blocking in Randomized Experiments

Randomized experiments are often performed to study the causal effects of interest. Blocking is a technique to precisely estimate the causal effects when the experimental material is not homogeneous. It involves stratifying the available experimental material based on the covariates causing non-homogeneity and then randomizing the treatment within those strata (known as blocks). This eliminates the unwanted effect of the covariates on the causal effects of interest. We investigate the problem of finding a stable set of covariates to be used to form blocks, that minimizes the variance of the causal effect estimates. Using the underlying causal graph, we provide an efficient algorithm to obtain such a set for a general semi-Markovian causal model.

==> sections-clear/abstract.tex <==
\begin{abstract}
    \textit{Randomized experiments} are often performed to study the causal effects of interest. \textit{Blocking} is a technique to precisely estimate the causal effects when the experimental material is not homogeneous. It involves stratifying the available experimental material based on the covariates causing non-homogeneity and then randomizing the treatment within those strata (known as \textit{blocks}). This eliminates the unwanted effect of the covariates on the causal effects of interest. We investigate the problem of finding a \textit{stable} set of covariates to be used to form blocks, that minimizes the variance of the causal effect estimates. Using the underlying causal graph, we provide an efficient algorithm to obtain such a set for a general \textit{semi-Markovian} causal model.
\end{abstract}


==> sections-clear/conclusion.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}
We have obtained a statistically optimal blocking set ($\textit{\textbf{Z}}^*$) such that it is the smallest subset of the observed covariates ($Z_1, \cdots, Z_n$) (excluding the forbidden ones) which will account (through blocking) for the maximum possible elimination of variability in response ($Y$). Further perspective on optimality is to prune a statistically optimal blocking set for economic reasons. For instance, suppose that we are restricted to creating blocks using at most $k$ covariates and a statistically optimal blocking set is of cardinality $>k$. One possible way to \textit{optimally} prune a statistically optimal blocking set is by dropping the covariates which are least significant in controlling the variability in response.
Or the question can be what is the minimum number of covariates required to eliminate as much as $(1-\alpha)\times 100 \%$ of the variability eliminated by a statistically optimal blocking set, for some user-defined $0\le\alpha\le1$. The idea is to do constrained optimization, where the constraint is usually a user-defined economic cost restriction.

Hence, we need to have a way to decompose the total variability controlled by a statistically optimal blocking set in terms of its individual elements, i.e., to quantify the contribution of each individual covariate in the optimal blocking set controlling the variability in the response. For the example graph in \cref{fig:figure7}, we have seen that a statistically optimal blocking set is $\textit{\textbf{Z}}^* = \{Z_1,Z_2,Z_3,Z_4\}$. We are interested in further pruning this set due to economic reasons. Note that, $Z_1$ and $Z_2$ are the parents of $Y$ and have direct effect on $Y$ through $Z_1 \rightarrow Y$ and $Z_2 \rightarrow Y$, respectively. $Z_4$ affects $Y$ through either of the routes viz., through $Z_4 \rightarrow Z_2 \rightarrow Y$ when $Z_2$ is unblocked, and through $Z_4 \rightarrow Z_2 \leftrightarrow Y$ when $Z_2$ is blocked. Similarly, $Z_3$ also affects $Y$ one of the two routes.

Suppose it is possible to quantify all the causal effects through the observed variables then we can take the following subgraph of \cref{fig:figure9} the with varying thickness of the edges between observed variables, where the thickness represents the strength of the link.

\begin{figure}[h!]
\centering
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10a}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->] (Z2) to node {} (Y);
  \draw[->,ultra thick] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10b}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->,ultra thick] (Z2) to node {} (Y);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10c}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->,ultra thick] (Z2) to node {} (Y);
  \draw[->,ultra thick] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10d}
\end{minipage}
\caption{Subgraphs of \cref{fig:figure9} involving $\{Z_4,Z_2,Y\}$ with varying link strengths.}
\end{figure}

In \cref{fig:figure10a} both the links are weak, hence we can discard both. In \cref{fig:figure10b} the link $Z_4 \rightarrow Z_2$ is strong but the strength of the effect of $Z_4$ on $Y$ through the path $Z_4 \rightarrow Z_2 \rightarrow Y$ depends on how strong the link $Z_2 \rightarrow Y$ is? It can be seen that in Figure 14(b) the link $Z_2 \rightarrow Y$ is weak which suggest that we can discard $Z_2$ and as long as we don't block $Z_2$ we never open the path $Z_4 \rightarrow Z_2 \rightarrow Y$, and hence we can discard $Z_4$ also. In \cref{fig:figure10c} the link  $Z_2 \rightarrow Y$ is strong which suggest that we should block $Z_2$. Blocking $Z_2$ will open the path the $Z_4 \rightarrow Z_2 \rightarrow Y$ but as the link $Z_3 \rightarrow Z_4$ is weak we can discard $Z_4$. In \cref{fig:figure10d} the link $Z_2 \rightarrow Y$ is strong which suggest that we should block $Z_2$. Blocking $Z_2$ will open the path the $Z_4 \rightarrow Z_2 \rightarrow Y$ and as the link $Z_3 \rightarrow Z_4$ is strong we should block $Z_4$ also.

The discussion can be used to motivate towards how and when further pruning of a statistically optimal blocking set can be done due to economic reasons. But there are several issues as follows.
\begin{enumerate}
\item Quantification of causal effects will require some observational data which may be difficult specifically for the treatment and response variables. Though all the covariates that we need to worry about are all pre-treatment and pre-response which are usually observed.
\item Even with the availability of some observational data for some or all variables, it may be possible that the causal effect is not identifiable.  
\end{enumerate}

In the case of some specific cases of linear models simple linear regression and Wright's rule can be of some help. But making some general statements is very difficult. For instance, the strength of the links $Z_4 \rightarrow Z_2$ and $Z_3 \rightarrow Z_4$ can be assessed by regressing $Z_4$ on $Z_2$, and $Z_3$ on $Z_1$.

In general, an economic restriction may not just be on the number of covariates to block using. As seen in the example in Section \ref{sec:challenges}, the economic cost of blocking depends also on the dimensionality of the covariates. Hence, one possible way to think about the economic cost of a blocking set is the resulting no. of blocks. But, the cost of a blocking set may not just be the no. of blocks. It can also involve how costly each covariate is otherwise. For instance, blocking using gender may be costlier than using age, though gender results in 2 blocks and age result in 4 blocks. Hence, the general definition of the economic cost of a blocking set should account for the resulting no. of blocks and the cost of forming those blocks for different covariates in that blocking set.


{\bf Some text needed}
\begin{definition}
The \textit{economic cost of a blocking set} is defined as a weighted sum of the dimensions of the covariates in it, where weights are their individual costs of forming blocks.
\end{definition} 
Note that, when all the covariates are equally costly and are of the same dimension, the cost of blocking is nothing but its cardinality, the case which we have considered at the beginning of this section.

{\bf Some text needed}
\begin{definition}
The \textit{statistical cost of a blocking set} is defined as the inverse of the amount of variability in the response that it controls for.
\end{definition}
Note that, we haven't completely addressed how to quantify the statistical cost of blocking.

{\bf Some text needed}
\begin{definition} \label{def:optimal_blocking_set}
The smallest subset of the set of observed covariates (excluding some forbidden variables if there are any) is said to be an \textit{optimal blocking set} if it minimizes the statistical cost of blocking among all the subsets of the set of observed covariates (excluding some forbidden variables if there are any), having an economic cost less than or equal to some user-defined threshold.
\end{definition} 

Developing an algorithm to obtain an optimal blocking set defined in Definition \ref{def:optimal_blocking_set} is an open problem that we aim to address in our future work.

==> sections-clear/extra.tex <==
There can be two types of causal effect that one might be interested in estimating, viz.,
\begin{enumerate}
    \item individual causal effect for the $i$th unit, i.e. the causal effect of $X_i$ on $Y_i$, and
    \item overall causal effect of $X$ on $Y$ 
\end{enumerate}

Let $Y_i$ be the response for the $i$th unit. Define the response for the $i$th unit when it receives the treatment as
\begin{align}
Y_{1i} &: = Y_i \text{ when } X_i=1.
\end{align}
Define the response for the $i$th unit when it does not receive the treatment as
\begin{align}
Y_{0i} &:= Y_i \text{ when } X_i=0.
\end{align}
\citet{rosenbaum1983central} termed $Y_{1i}$ and $Y_{0i}$ as \textit{potential outcomes} for the $i$th unit when it receives the treatment and when it is under control, respectively. 

For the $i$th unit, we can define the causal effect of the treatment as the difference between the potential outcomes under treatment and control, i.e., $Y_{1i}-Y_{0i}$. However, individual treatment effects cannot be calculated as we only observe $X_i$ and $Y_i = X_iY_{1i} + (1-X_i)Y_{0i}$ \citep{holland1986statistics}, which is due to the fact that we don't assign treatment to all the units rather we randomize. Because of this missing data problem, attention has been focused on some parameters which can summarize the causal effect, usually in terms of expectations. Following \citep{heckman1992randomization}, \citep{clements1994making}, and \citep{heckman1995assessing}, we define the \textit{effect of treatment} (ET) in the population as
\begin{align}
\beta = E(Y_{1}-Y_{0}), \text{ and}
\intertext{the \textit{effect of treatment on treated} (ETT) in the population as}
\gamma = E((Y_{1}-Y_{0})|X=1).
\end{align}

We focus on estimation of $\beta = E(Y_{1}-Y_{0})$. We introduce the following notations.
\begin{align*}
    I_1 &= \{i:X_i=1\}, \ n_1 = |I_1|,\\
    I_0 &= \{i:X_i=0\}, \ n_0 = |I_0|.
\end{align*}

The natural non-parametric estimate of this expectation is the corresponding sample average, and is given as
\begin{align}
\hat{\beta} &= \frac{1}{n_1}\sum_{i:X_i=1}Y_{1i}-\frac{1}{n_0}\sum_{i:X_i=0}Y_{0i} \nonumber \\ 
&:= \bar{Y}_1 - \bar{Y}_0. \label{def:sample_mean}
\end{align}

$E(\hat{\beta}) = \beta$, i.e., $\hat{\beta}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}$ (normalized for sample size) is given as follows.
\begin{align}
    V(\hat{\beta}) = 
      E_Z\bigg(\frac{V(Y_1|Z)}{P(X=1|Z)} &+ \frac{V(Y_0|Z)}{P(X=0|Z)} \nonumber \\ &\text{} + (\beta(Z)-\beta)^2 \bigg) \label{eq:var_under_no_blocking}
\end{align}

% \begin{align}
%     V(\hat{\beta}) & = 
%     \begin{cases}
%       E_Z\left(\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  + (\beta(Z)-\beta)^2 \right), & \text{under non-homogeneity},\\
%       \frac{V(Y_1)}{P(X=1)} + \frac{V(Y_0)}{P(X=0)}, &  \text{under homogeneity}. \tag{2} \label{eq:var_under_no_blocking}
%     \end{cases}
% \end{align}

Prior works \citep{} suggest to do blocking in the situation when the experimental units are not homogeneous. Let us see how does the estimator $\hat{\beta}$ defined in Equation \ref{def:sample_mean} should be updated, under blocking using covariates in $Z$. Following Theorem \ref{} of \citep{petersen2006estimation}, we have
\begin{align}
\beta &= E(Y_{1}-Y_{0}) = E_Z\left(E((Y_{1}-Y_{0})|Z)\right), \nonumber\\ 
&= E_Z\left(E(Y_{1}|Z)-E(Y_{0}|Z)\right) \nonumber \\ 
&= \sum_{Z=z}\left(E(Y_{1}|Z=z)-E(Y_{0}|Z=z)\right)P(Z=z).
\end{align}
Hence, we can define an estimator of $\beta$ under blocking using covariates in $Z$, as follows.
\begin{align}
\hat{\beta}_Z & = \sum_{Z=z}\left(\hat{E}(Y_{1}|Z=z)-\hat{E}(Y_{0}|Z=z)\right)\hat{P}(Z=z), \nonumber \\
&= \sum_{Z=z}\left((\bar{Y_{1}}|Z=z)-(\bar{Y_{0}}|Z=z)\right)\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)},
\end{align}
where $\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)}$ is the proportion of units in the block formed with characteristics $Z=z$.

Suppose there are no units in one or more blocks, i.e., $\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)} = 0$ for some $z$, then the overall average treatment effect can be estimated but the $z$-specific causal effect cannot be estimated. Hence, it is desirable to have units in every block. This also rules out the argument against randomized block experiments that matching of units can be done post a completely randomized experiment based on the covariates, as it is possible that there are no units corresponding to a particular covariate combination.

$E(\hat{\beta}_Z) = \beta$, i.e., $\hat{\beta}_Z$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}_Z$ (normalized for sample size) is given as follows.
\begin{align}
    V(\hat{\beta}_Z) = E_Z\bigg(&\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  \nonumber \\  &\text{ } + \big(\sum_Z\beta(Z)\hat{P}(Z) - \beta \big)^2 \bigg) \label{eq:var_under_blocking}
\end{align}
% \begin{align}
%     V(\hat{\beta}_Z) & = 
%     \begin{cases}
%       E_Z\left(\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  + \left(\sum_Z\beta(Z)\hat{P}(Z) - \beta \right)^2 \right), & \text{non-homogeneity},\\
%       \frac{V(Y_1)}{P(X=1)} + \frac{V(Y_0)}{P(X=0)}, &  \text{homogeneity}.
%     \end{cases} \tag{4} \label{eq:var_under_blocking}
% \end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gain in Precision due to Blocking}
Consider a simple setting where $X$ is an indicator random variable defined as
\begin{equation}
X = 
\begin{cases} 
    1, & \text{if the treatment is applied}, \\
    0, & \text{otherwise,}
\end{cases}
\end{equation}
and $Y$ is real-valued random variable.

Let there be $n$ experimental units available to study the causal effect of $X$ on $Y$ by performing a randomized experiment. Let $\mathcal{Z}$ denote the set of covariates that vary across the experimental units. 

We want to demonstrate the gain in precision due to blocking. Hence, we first ignore these covariates and perform a CRD as follows. We randomize $X$ over the available experimental units, i.e. randomly assign a unit to either have the treatment ($X=1$) or not ($X=0$), and then observe the response. Let $(X_i,Y_i)$ denote the treatment and response pair for the $i$th experimental unit. %As different units are identical and we have randomized the treatment, $X_i$ and $Y_i$ are nothing but i.i.d. copies of $X$ and $Y$, respectively. In other words, $\{(X_i,Y_i): i=1,\dots,n\}$ is a random sample from ($X,Y$). 
Define $I_x:=\{i:X_i=x\}$ and $n_x:=|I_x|$. 

%denote the set of indices of units where the value of treatment, and $I_1:=\{i:X_i=0\}$ denote the set of indices of units where the treatment is not applied. Further, define $n_1:=|I_1|$ and $n_0:=|I_0|$.

We are interested in estimating $\mathbb{E}(Y|do(X))$. For simplicity, define $Y(x) := Y|do(X=x)$. For our simple setting, we have only two possibilities of the that conditional expectation, viz. $\mathbb{E}(Y(1))$ and $\mathbb{E}(Y(0))$.  Similar to \citep{heckman1992randomization}, \citep{clements1994making}, and \citep{heckman1995assessing}, we define the \textit{effect of treatment} (ET) in the population as
\begin{align}
\beta := \E(Y(1)) - \E(Y(0)). \label{eq:beta}
\end{align}
A natural non-parametric estimator of $\E(Y(x))$ is the corresponding sample average, given as
\begin{align}
\bar{Y}(x) &:= \frac{1}{n_x}\sum_{i\in I_x}Y_{i}.
\end{align}
Hence, we can estimate $\beta$ as
\begin{align}
\hat{\beta} &= \bar{Y}(1) - \bar{Y}(0)
\end{align}

It can be shown that $\mathbb{E}(\hat{\beta}) = \beta$, i.e., $\hat{\beta}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{\P(X=1|\mathcal{Z})} + \frac{\Var(Y(0)|\mathcal{Z})}{\P(X=0|\mathcal{Z})} \right) \nonumber \\ 
      \text{} + \mathbb{E}_\mathcal{Z}\left((\beta(\mathcal{Z})-\beta)^2 \right), \label{eq:var_under_no_blocking}
\end{align}
where $\beta(\mathcal{Z}):= \E(Y(1)|\mathcal{Z}) - \E(Y(0)|\mathcal{Z})$ is the $\mathcal{Z}$-specific causal effect. For proofs of unbaisedness and variance of $\hat{\beta}$, see Appendix.

We now perform an RBD as follows. We first stratify the experimental units such that units with each stratum (known as block) are identical, i.e. the covariates in $\mathcal{Z}$ remain same with a block. We next randomize $X$ over the experimental units within each block, and then observe the response. Let $(X_i,Y_i,\mathcal{Z}_i)$ denote the treatment, response, and covariates triplet for the $i$th experimental unit. Define $I_{x,z}:=\{i:X_i=x,\mathcal{Z}_i = z\}$ and $n_{x,z}:=|I_{x,z}|$. 

Note that ET defined in \eqref{eq:beta} can be re-written as \citep{petersen2006estimation}
\begin{align}
    \beta &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}\right) - \E_\mathcal{Z}\left(\E(Y(0) | \mathcal{Z}\right), \nonumber\\
    &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}) - \E(Y(0) | \mathcal{Z})\right), \nonumber\\
    &= \sum_{\mathcal{Z} = z} \left(\E(Y(1) | \mathcal{Z}=z) - \E(Y(0) | \mathcal{Z}=z) \right) \P(\mathcal{Z}=z) \label{eq:beta_z}
\end{align}
A natural non-parametric estimator of $\E(Y(x)|\mathcal{Z}=z)$ is the corresponding sample average, given as
\begin{align}
    \bar{Y}(x)|(\mathcal{Z}=z) &:= \frac{1}{n_{x,z}}\sum_{i\in I_{x,z}} Y_i
\end{align}
$\P(\mathcal{Z}=z)$ can be estimates as
\begin{align}
    \hat{\P}(\mathcal{Z}=z) &:= \frac{n_{x,z}}{n}
\end{align}
Hence, we can estimate $\beta$ as
\begin{align}
\hat{\beta}_\mathcal{Z} &= \frac{1}{n}\sum_{\mathcal{Z} = z} n_{x,z} \left(\bar{Y}(1) | (\mathcal{Z}=z) - \bar{Y}(0) | (\mathcal{Z}=z) \right)
\end{align}
It can be shown that $\mathbb{E}(\hat{\beta}_\mathcal{Z}) = \beta$, i.e., $\hat{\beta}_\mathcal{Z}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}_\mathcal{Z}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}_\mathcal{Z}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{\P(X=1|\mathcal{Z})} + \frac{\Var(Y(0)|\mathcal{Z})}{\P(X=0|\mathcal{Z})} \right) \nonumber \\ 
      \text{} + \mathbb{E}_\mathcal{Z} \left(\left(\sum_{\mathcal{Z}=z}\beta(\mathcal{Z}=z)\hat{\P}(\mathcal{Z}=z) - \beta \right)^2\right), \label{eq:var_under_blocking}
\end{align}
For proofs of unbaisedness and variance of $\hat{\beta}_\mathcal{Z}$, see Appendix.

By comparing \eqref{eq:var_under_no_blocking} and \eqref{eq:var_under_blocking}, we observe that $\Var(\hat{\beta}_\mathcal{Z}) \le \Var(\hat{\beta})$, i.e. blocking improves the precision of the estimate of the population average causal effect, $\beta$.

%Another example to demonstrate the gain in precision due to blocking is as follows. Suppose there are $k$ treatments and $b$ blocks, then the response can be defined as a linear equation: $y_{ij} = \mu + \tau_i + b_j + \epsilon_{ij}$, where $\mu$ is the general mean effect, $\tau_i$ is the effect due to the the $i$th treatment, $b_j$ is the effect due to the $j$th block, and $\epsilon_{ij}$ is the noise or the experimental error. Clearly, in the absence of $b_j$, error is higher as compared to the case when $b_j$ is there.

%If the experimental units are identical then $\hat{\beta}_\mathcal{Z} = \hat{\beta}$. 

%\textbf{Remark.} Suppose there are no units in one or more blocks, i.e., $n_{x,z} = 0$ for some $z$, then the overall average treatment effect can be estimated but the $z$-specific causal effect cannot be estimated. Hence, it is desirable to have units in every block. This also rules out the argument against randomized block experiments that matching of units can be done post a completely randomized experiment based on the covariates, as it is possible that there are no units corresponding to a particular covariate combination.

%\subsection{Gain in Precision under Blocking} We have seen that blocking improves the precision of the estimates. Sometimes, the interest is to study the causal effects from the observational data, possibility because carrying out a randomized experiment is either economically or ethically infeasible. An approach similar to blocking (in randomized experiments) called \textit{matching} is used to study the causal effects from the observational data, where grouping of units is done on covariates after getting the observational data. There covariate adjustment is done to reduce the confounding bias. For instance, \citep{rosenbaum1983central} provided a way to create blocks by matching the observation on propensity score, which is a famously termed as \textit{propensity score matching} (PSM). General concerns with matching have been raised by \citet{pearl2009causality}, who has argued that hidden bias may actually increase because matching on observed variables may unleash bias due to dormant unobserved confounders. Similarly, \citet{pearl2009causality} has argued that bias reduction can only be assured (asymptotically) by modeling the qualitative causal relationships between treatment, outcome, observed and unobserved covariates. Confounding occurs when the experimenter is unable to control for alternative, non-causal explanations for an observed relationship between independent and dependent variables. Such control should satisfy the \textit{back-door criterion} \citep{pearl2009causality}.



\begin{figure}[th]
\centering
\begin{minipage}{.49\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \end{scope}
\end{tikzpicture}
\caption{Example Markovian model.} \label{fig:figure1}
\end{minipage}
\begin{minipage}{.49\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize  $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \end{scope}
\end{tikzpicture}
\caption{Example semi-Markovian model with latent variables involving only covariates.} \label{fig:figure2}
\end{minipage}
\end{figure}

==> sections-clear/introduction.tex <==
\section{Introduction}

\subsection{Motivation}
Studying the \textit{causal} effect of some variable(s) on the other variable(s) is of common interest in social sciences, computer science, and statistics. However, a mistake that people usually make is, confusing the causal effect with an \textit{associational} effect. For instance, if high levels of bad cholesterol and presence of a heart disease are observed at the same time, it does not mean that the heart disease is caused by the high levels of bad cholesterol. The question is then how do we get to know if at all a variable causes the other? If the answer is yes, then what is the direction (positive or negative) and what is the magnitude, of the causal effect? \cite{fisher1992statistical} provided the framework of \textit{randomized experiments} to study the causal effect, where the variable whose causal effect is to be studied (known as \textit{treatment} or cause), is randomized over the available experimental material like humans, rats, agricultural plots etc. and changes in the variable on which the causal effect is to be studied  (known as \textit{response} or effect), are recorded. A statistical comparison of values of the response with or without the treatment can therefore be done to study the existence, direction and magnitude of the cause-effect relationship of interest.

Randomized experiments work on three basic principles, viz., \textit{randomization}, \textit{replication}, and \textit{local control}. Randomization states that the assignment of the treatment has to be random, replication states the treatment should be given to multiple but homogeneous units, i.e., there are multiple observations of the effect variable for both with and without the treatment. Hence, as long as the entire experimental material is homogeneous (for instance, the fertility of all the agricultural plots is same, the responsiveness of all the humans is same for the drug, etc.), then a `good' randomized experiment can be carried out using the first two principles, viz., randomization and replication, which gives rise to  \textit{completely randomized design} (CRD). However, when the entire experimental material is not homogeneous, i.e., some attributes of experimental units (known as \textit{covariates}) differ from each other, then the causal effect may get influenced by the covariates causing non-homogeneity like fertility, responsiveness, etc. The remedy to this problem is the third principle of randomized experiments, i.e., local control (also known as \textit{blocking}), which states to stratify the entire experimental material based on that covariate(s) causing non-homogeneity, and then randomize the treatment within those strata to eliminate the effect of the covariates. These strata are called \textit{blocks}, and this third principle along with the first two give rise to  \textit{randomized block design} (RBD). Blocking tries to control/eliminate the variability in the response attributed through the covariates and leads to a more \textit{precise} estimation of the caual effect of interest. %Precision is defined as inverse of the variability which measures how much the response would have varied if the sample would have changed. In the context of estimating the causal effects, precision is  the inverse of the variance of the estimate of the causal effect. 

In this paper, we focus on the problem of deciding which covariates to use for creating the blocks while performing a randomized experiment. We consider a non-parametric setting and assume that we have access to the underlying structural causal model \cite{pearl2009causality}. We provide a graphical criterion to obtain a statistically optimal set of covariates to use for creating the blocks for a general semi-Markovian causal graph.

\subsection{Literature Review}
Statistics literature \cite{yates1935complex}, \cite{kempthorne1952design}, \cite{kempthorne1955randomization}, \cite{cochran1948experimental} presents profound discussions on relative efficiency (ratio of the variances of causal effects) of RBD over CRD. It can be seen that in general, RBD is always more or at least as efficient as CRD. Hence, the natural question is how do we do blocking in an intelligent manner such that maximum gain in precision can be attained, i.e., variability in the response due to the covariates, can be controlled to a maximum possible extent? More specifically, we are interested in knowing which all covariates should be used to create blocks? Intuitively, we can say that we need not take the ones into consideration which remain constant in the population. But, among the ones which vary, can we choose some over the other, using some criterion? 

Most of the blocking schemes discussed in the literature discuss about creating blocks by grouping the experimental units which are close to each other based on some attributes. For instance, \textit{threshold blocking} \cite{higgins2016improving}.

The question that we are interested in answering is, can we decide which covariates to use for creating blocks using the causal structure (diagram) of the all the variables, viz., treatment, response and covariates (observed and unobserved), provided the causal structure is given?

\subsection{Contribution}
The main contributions of this paper can be summarized as follows.
\begin{enumerate}
    \item We formalize the problem of obtaining a statistically optimal set of covariates to be used to create blocks in randomized experiments under a non-parametric setting.
    \item We provide a graphical test to obtain such a set for a general semi-Markovian causal model. 
    %\item We also propose and provide ideas towards solving a more general problem of obtaining an optimal blocking set that considers both the statistical and economic costs of blocking.
\end{enumerate}

\subsection{Organization}
The rest of the paper is organized as follows. \Cref{sec:prob_formulation} provides some background and formulates the problem of interest. \Cref{sec:methodology} first discusses some key observations and motivating examples, and then provides the main results. \Cref{sec:conclusion} concludes the paper and provides future directions.

==> sections-clear/methodology.tex <==
\section{Methodology} \label{sec:methodology}
In this section, we develop a methodology to find a solution to \cref{problem:optimal_blocking}. We first examine $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$ to obviate some edges and nodes from the causal graph, $\mathcal{G}$. We next discuss some motivating examples and make key observations that lead to several lemmas for our main result. In the end, we provide our main result and develop an efficient algorithm for solving \cref{problem:optimal_blocking}.

\subsection{Examining $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$}
In \cref{problem:optimal_blocking}, our interest is to minimize $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}\subseteq \mathcal{C}$. $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ through the causal relationships from $\mathcal{Z}$ to $Y$, and from $\mathcal{Z}$ to $X$. Note that, $X$ is the treatment on which we are performing the intervention, i.e.,  we set the levels/values of $X$. This is equivalent to saying that $X$ is no longer affected by the rest of the variables. Therefore, $\mathcal{Z}$ also cannot affect $X$ when an intervention is performed on $X$. %instead its value is decided/set during the experiment. %In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all arrows coming into $X$. 
Therefore, $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from $\mathcal{Z}$ to $Y$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}$ to $Y$ gives a solution to \ref{problem:optimal_blocking}.

Denote the subgraph of $\mathcal{G}$ where all edges coming into $X$ were deleted as $\mathcal{G}_{\widetilde{X}}$.
\begin{lemma} \label{lemma:Gxbar}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}_{\widetilde{X}}$.
\end{lemma}
\begin{proof}
The proof follows from the fact that when an intervention is performed on $X$ then it is no longer affected by the rest of the variables. In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all edges coming into $X$. 
\end{proof}

\begin{definition}
$\mathcal{S},\mathcal{T}\subseteq \mathcal{C}$ are called equivalent sets (denoted as $\mathcal{S} \equiv \mathcal{T}$), if  $\Var(\hat{\P}_\mathcal{S}(Y|do(X))) = \Var(\hat{\P}_\mathcal{T}(Y|do(X)))$.
\end{definition}

\begin{lemma} \label{lemma:D0}
If $\mathcal{F}$ is the set of all covariates that do not have causal paths to $Y$, then $\mathcal{C}$ and $\mathcal{C}\backslash \mathcal{F}$ are equivalent sets.
\end{lemma}
\begin{proof}
The proof follows from the fact that a set of covariates can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from itself to $Y$.
\end{proof}
Following \cref{lemma:Gxbar}, we restrict ourselves to the subgraph $\mathcal{G}_{\widetilde{X}}$. Following \cref{lemma:D0}, we further delete the covariates that do not have any causal paths to $Y$. Denote this new subgraph as $\mathcal{G}'_{\widetilde{X}}$ and $\mathcal{C}'=\mathcal{C}\backslash\mathcal{F}$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}'$ to $Y$ in $\mathcal{G}'_{\widetilde{X}}$ gives a solution to \ref{problem:optimal_blocking}.

%As discussed earlier, we are interested in performing a randomized experiment to study the causal effect of interest $X\rightarrow Y$ where we are randomizing the treatment $(X)$. In terms of the causal graph, randomizing $X$ is the same as making interventions to set levels/values of $X$. This means that $X$ is not affected by any variable in the graph, instead, its value is decided/set during the experiment. Therefore, we can \textit{ignore all the arrows coming into $X$} and work with the subgraph of $G$ where all arrows coming into $X$ are ignored. We denote such subgraph as $G_{\widetilde{X}}$. Therefore, for the examples, we work with causal graphs with no arrows coming to $X$.

\subsection{Motivating Examples and Key Observations}

All causal graphs in \cref{fig:markovian_model,fig:semi_markovian_model_C,fig:semi_markovian_model_Y,fig:semi_markovian_model_des,fig:semi_markovian_model_postx} represent represent $\mathcal{G}'_{\widetilde{X}}$. Denote the set of parents of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{P}(W)$.

\textbf{Note.} In all the graphs provided in this paper, a bi-directed edge between any two observed variables is same as those two variables having one or more unobserved ancestors. For example $V_3 \xdashleftrightarrow V_4$.

\textbf{Example 1.} For \cref{fig:markovian_model,fig:semi_markovian_model_C}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. Therefore, $\mathcal{Z}^* = \mathcal{P}(Y)\backslash\{X\}$.
\begin{figure}[th]
\centering
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \end{scope}
\end{tikzpicture}
\caption{Example Markovian model (no latent structures).} \label{fig:markovian_model}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize  $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \end{scope}
\end{tikzpicture}
\caption{Example semi-Markovian model with latent variables involving only $\mathcal{C}'$.} \label{fig:semi_markovian_model_C}
\end{minipage}
\end{figure}

\textbf{Example 2.} For \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is not sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. In \cref{fig:semi_markovian_model_Ya}, the reason is that blocking using $V_2$ opens the path $V_4 \rightarrow V_2 \leftarrow Y$ for $V_4$ to cause variability in $Y$. In \cref{fig:semi_markovian_model_Yb}, the reason is that the latent structure $Y \leftrightarrow V_4$ enables $V_4$ to cause $Y$ even when the path $V_4\rightarrow V_2\rightarrow Y$ is blocked. For both \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{Z}^*=(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$.
\begin{figure}[thb]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Ya}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Yb}
\end{minipage}\hspace{.5cm}
\caption{Example semi-Markovian model with latent variables involving $\mathcal{C}'$ and $Y$.}\label{fig:semi_markovian_model_Y}
\end{figure}

\textbf{Example 3.} For \cref{fig:semi_markovian_model_des}, despite $Y$ having descendants, $(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. This is because descendants of $Y$ can never be a cause of variability in $Y$. In \cref{fig:semi_markovian_model_desa,fig:semi_markovian_model_desb}, $V_5$ (a descendant of $Y$) cannot cause $Y$ through the edge $Y \rightarrow V_5$. Moreover, $V_4$ (an ancestor of $Y$) cannot cause $Y$ through $V_5$ because $V_5$ is a collider on the path $V_4\rightarrow V_5 \leftarrow Y$.

\begin{figure}[th]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[->, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desa}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desb}
\end{minipage}
\caption{Example Semi-Markovian Models with latent variables involving $\mathcal{C}'$ and $Y$, and $Y$ having descendants.}\label{fig:semi_markovian_model_des}
\end{figure}

Denote the set of ancestors (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{A}(W)$. Denote the subgraph of $\mathcal{G}'_{\widetilde{X}}$ restricted to $\mathcal{A}(Y)$ as $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Based on the insights from Examples 1 to 3, we write the following lemma.
\begin{lemma}\label{lemma:GxbarA}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$.
\end{lemma}

\begin{proof}
The proof follows from the fact that the descendants of a node can never be its cause even in the presence of latent structures.
\end{proof}

\subsection{Solution to Problem \ref{problem:optimal_blocking}}

We now combine the insights from \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA} to provide a solution to \cref{problem:optimal_blocking}.

\begin{theorem} \label{theorem:sol_to_optimal_blocking}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ is a solution to \cref{problem:optimal_blocking}.
\end{theorem}
\begin{proof}
The proof follows from the fact that $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. %following \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA}.
\end{proof}

\cref{theorem:sol_to_optimal_blocking} provides a sufficient condition for a set $\mathcal{Z}$ to be a solution to \cref{problem:optimal_blocking}. We next provide a method to construct a set $\mathcal{Z}$ that satisfies this sufficient condition.

Let a path composed entirely of bi-directed edges be called a \textit{bi-directed path}.
\begin{definition}\label{def:c_component} \citep{tian2002general}. 
For a graph $\mathcal{G}$, the set of observed variables $\mathcal{V}$, can be \textit{partitioned} into disjoint groups by assigning two variables to the same group if and only if they are connected by a bi-directed path. Assume that $V$ is therefore partitioned into $k$ groups $\mathcal{S}_1, \dots, \mathcal{S}_k$. We will call each $\mathcal{S}_j; j=1, \dots, k,$ a \textit{$c$-component} of $V$ in $\mathcal{G}$ or a $c$-component (abbreviating confounded component) of $\mathcal{G}$. The $\mathcal{S}_j$ such that $W\in S_j$ is called the \textit{$c$-component of $W$} in $\mathcal{G}$ and is denoted as $C_{W,\mathcal{G}}$. As $\{\mathcal{S}_1, \dots, \mathcal{S}_k\}$ is a partition of $\mathcal{V}$, $c$-component of a variable always exists and is unique.
\end{definition}

In Example 2, we observed that due to the presence of latent structures involving $Y$, $\mathcal{P}(Y)$ was not sufficient to block all causal paths from $\mathcal{C}'$ to $Y$. However the parents of $c$-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ would be sufficient for that purpose. 

\begin{theorem} \label{theorem:sol_to_optimal_blocking_construction}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ is  the set of parents of c-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ excluding $X$ denoted as $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$.
\end{theorem} 
\begin{proof}
The proof follows from Corollary 1 \citep{tian2002studies}, which states that a node is independent of its ancestors excluding the parents of its $c$-component given the parents of its $c$-component.
\end{proof} 

\textbf{Note.} In a Markovian model there are no bi-directed paths, Therefore, the elementary partition of $\mathcal{A}(Y)$ is the $c$-component of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Therefore, $C_Y = \{Y\}$, and $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}) \backslash\{X\} = \mathcal{P}(Y) \backslash\{X\}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. This matches with our insight in Example 1, where we saw that $Y \perp (\mathcal{A}(Y)\backslash\{X,Y\})\backslash(\mathcal{P}(Y)\backslash\{X\})|(\mathcal{P}(Y)\backslash\{X\})$.

\subsection{Stability of the Solution to Problem \ref{problem:optimal_blocking}} \label{sec:stable_blocking}

We next discuss some concerns with using $\mathcal{Z}^*$ (a solution to \cref{problem:optimal_blocking}) as a blocking set. We provide a method to address those concerns. 

\textbf{Example 4.} In \cref{fig:semi_markovian_model_postxa} and \cref{fig:semi_markovian_model_postxb}, there are some covariates which are ancestors of $Y$ and descendants of $X$. Such covariates are called post-treatment ancestors (excluding itself) of the response. Blocks created using these covariates are not well-defined. For instance, we are interested in studying the causal effect of a drug on blood pressure. Suppose anxiety level mediates the effect of drug on blood pressure, i.e., $\text{drug}\rightarrow\text{anxiety}\rightarrow \text{blood pressure}$. If we create blocks using anxiety then the blocks will change (i.e., become unstable) during the experiment because change in the drug level will cause the anxiety level to change. Therefore, it is reasonable not to create blocks using these covariates. With this insight, for \cref{fig:semi_markovian_model_postxa}, $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_4\}$ blocks all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$. 

However, we cannot simply delete the post-treatment ancestors (excluding itself) of the response from the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ of interest. This is because the presence of latent structures between pre- and post-treatment ancestors of the response affects blocking set of interest. For instance, in \cref{fig:semi_markovian_model_postxb}, $V_1$ is a collider on the path $V_3\rightarrow V_1\leftarrow V_6$. Hence, keeping $V_1$ in the blocking set will open this path for $V_3$ to cause variability in $Y$. Therefore, for  \cref{fig:semi_markovian_model_postxb}, we need $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_3,V_4\}$ to block all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$.

\begin{figure}[t]
\centering
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxa}
\end{minipage}
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend right] (Z1) to node {} (Z6);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxb}
\end{minipage}
\caption{Example semi-Markovian models with post-treatment ancestors of $Y$.}\label{fig:semi_markovian_model_postx}
\end{figure}

% To formalize the insight from Example 4, we refer to the following definition.
% \begin{definition} \cite{shpitser2012validity} A causal path from a variable $X \in \mathcal{X}$ to $Y \in \mathcal{Y}$ is called \textit{proper} if it doesn't intersect $\mathcal{X}$ except the endpoints. When $\mathcal{X}$ is a single variable then all causal paths are proper.
% \end{definition}

Denote the post-treatment ancestors (excluding itself) of the response while studying the causal effect $Y|do(X)$ as $\mathcal{M}(Y|do(x))$.
\begin{definition}
For studying the causal effect of $X$ on $Y$, a blocking set $\mathcal{Z}$, is said to be stable if $\mathcal{Z} \cap \mathcal{M}(Y|do(x)) = \phi$.
\end{definition}

Denote the set of descendants (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ as $\mathcal{D}(\cdot)$. %Denote the set of ancestors of $W$ in the subgraph of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ where all edges leaving $X$ as $\mathcal{A}$.
\begin{lemma} \label{lemma:M}
$\mathcal{M}(Y|do(x)) = (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
\end{lemma}
\begin{proof}
The proof follows from the definition of post-treatment ancestors (excluding itself) of $Y$.
\end{proof}

\begin{theorem}\label{theorem:stable_blocking}
A stable solution to \cref{problem:optimal_blocking} is $\mathcal{Z}^* = (\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}} \backslash\{X\}) \backslash \mathcal{M}(Y|do(x))$.
\end{theorem}
\begin{proof}
The proof follows from \cref{lemma:M}.
\end{proof}

%Therefore, we ignore all the variables falling on a proper causal path from $X$ to $Y$. Following \cite{van2014constructing}, the set of all such variables is $Dpcp(X,Y) = De((De_{\widetilde{X}}(X) \backslash X) \cap An_{\tilde{\tilde{X}}(Y))$ where $De(.)$ represents the set of descendants excluding the variable itself and $An_{\tilde{\tilde{X}}(Y)}$ is the ancestral graph of $Y$ where all edges leaving $X$ are removed.

%Note that by definition $Dpcp(X,Y)$ may include non-descendants of $Y$ which we have already argued to not take into consideration in Observation 2. Therefore, we can say that specifically we should not block using  $Dpcp(X,Y)$ in the graph $G_{An_{\widetilde{X}}(Y)}$ denoted as $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}}$. Note that $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}} = Dpcp(X,Y) \cap An_{\widetilde{X}}(Y)$.

\subsection{Final Algorithm}

We next provide steps to obtain a stable solution to \cref{problem:optimal_blocking} based on \cref{theorem:sol_to_optimal_blocking,theorem:sol_to_optimal_blocking_construction,theorem:stable_blocking}. First, we reduce $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Next, we obtain the set $\mathcal{Z} = \mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$ which is the smallest set such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Finally, we drop $\mathcal{M}(Y|do(x))$ from $\mathcal{Z}$ to get a stable solution to \cref{problem:optimal_blocking}.

Denote the edge $W_1\rightarrow W_2$ as \textit{directed-edge}$(W_1,W_2)$, a path consisting of directed edges from $W_1$ to $W_2$ as \textit{directed-path}$(W_1,W_2)$, and a path consisting of all bi-directed edges from $W_1$ to $W_2$ as \textit{bi-directed-path}$(W_1,W_2)$. Algorithm \ref{alg:causal-opt-blocking-set} outlines the psuedocode of the proposed algorithm to obtain a stable solution to \cref{problem:optimal_blocking}.

\begin{algorithm} [!htb]
	\caption{Stable-Causal-Blocking ($\mathcal{G}, X, Y$)}\label{alg:causal-opt-blocking-set}
	\begin{algorithmic}[1]
	    %\State \textbf{Input} {($\mathcal{G}, X, Y$)}.
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}$ to $\mathcal{G}_{\widetilde{X}}$} 
            \If{$\exists$ \textit{directed-edge}($V_i,X$)}
                \State delete \textit{directed-edge}($V_i,X$) from $\mathcal{G}$
            \EndIf
        \EndFor 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X}}$} 
            \If{$\nexists$ \textit{directed-path}($V_i,Y$)}
                \State delete $V_i$ from $\mathcal{G}$
            \EndIf
        \EndFor 
        \State $\mathcal{A}'(Y) \leftarrow \phi$
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}'_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$} 
        \If{$\nexists$ path($V_i,Y$)}
            \State delete $V_i$ from $\mathcal{G}; \mathcal{A}'(Y) \leftarrow \mathcal{A}'(Y) \cup \{V_i\}$
        \EndIf
        \EndFor
        \State $\mathcal{A}(Y) = \mathcal{V}\backslash\mathcal{A}'(Y)$
        \State $\mathcal{S}_i = \{V_i\}, i =1,\dots,|\mathcal{V}|$ \Comment{Finding $C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$}
            \For{$j$ in $1,\dots,i$}
            \If{$\exists$ \textit{bi-directed-path}($V_i$,$V_j$)}
                \State $\mathcal{S}_i \leftarrow \mathcal{S}_i \cup \mathcal{S}_j; \mathcal{S}_j \leftarrow \phi$
            \EndIf
            \EndFor
        \EndFor
        \State $i\leftarrow 1; \mathcal{S} \leftarrow \mathcal{S}_1$
        \While{$Y \notin \mathcal{S}$} 
            \State $i \leftarrow i+1; \mathcal{S} \leftarrow \mathcal{S}_i$
        \EndWhile
        \State $\mathcal{P}(\mathcal{S})=\phi$ \Comment{Finding $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
            \For{$W$ in $\mathcal{S}$}
                \If{$\exists$ \textit{directed-edge}($V_i,W$)}
                    \State $\mathcal{P}(\mathcal{S}) \leftarrow \mathcal{P}(\mathcal{S}) \cup \{V_i\}$
                \EndIf
            \EndFor
        \EndFor 
    	\State $\mathcal{D}(X) \leftarrow \phi$ \Comment{Finding $\mathcal{D}(X)$} 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
        \If{$\nexists$ \textit{directed-path}($X,V_i$)}
            \State $\mathcal{D}(X) \leftarrow \mathcal{D}(X) \cup \{V_i\}$
        \EndIf
        \EndFor    	
    	\State $\mathcal{Z} \leftarrow (\mathcal{P}(\mathcal{S})\backslash\{X\}) \backslash (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
    	\State \textbf{return} $\mathcal{Z}$
	\end{algorithmic}
\end{algorithm}

\subsection{Time Complexity of Algorithm \ref{alg:causal-opt-blocking-set}}
We next show that \cref{alg:causal-opt-blocking-set} is an efficient polynomial-time algorithm. Finding if there exists a path between any two nodes in a directed graph can be done using breath-first-search which has the worst-case time complexity of $O(|\mathcal{V}|^2)$. \cref{alg:causal-opt-blocking-set} first reduces $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ which involves
\begin{enumerate}
    \item finding variables with edges going into $X$: $O(|\mathcal{V}|)$, 
    \item finding variables with no path into $Y$: $O(|\mathcal{V}|^3)$, and 
    \item finding all ancestors of $Y$: $O(|\mathcal{V}|^3)$.
\end{enumerate}
 
\cref{alg:causal-opt-blocking-set} next finds the $c$-component of $Y$ involves traversing all pairs of variables: $O(|\mathcal{V}|^2)$, and finding if there exists a bi-directed path between any pair of variables: $O(|\mathcal{V}|^2)$. Therefore, the total time at this step is $O(|\mathcal{V}|^4)$. Finally \cref{alg:causal-opt-blocking-set} finds $\mathcal{M}(Y|do(x))$ which involves
\begin{enumerate}
    \item finding descendants of $X$: $O(|\mathcal{V}|^3)$, and
    \item finding ancestors of $Y$: $O(|\mathcal{V}|^3)$.
\end{enumerate}

Therefore, the time complexity of \cref{alg:causal-opt-blocking-set} is $O(|\mathcal{V}|^4)$.

\subsection{Implementing Algorithm \ref{alg:causal-opt-blocking-set}}
We demonstrate the implementation of \cref{alg:causal-opt-blocking-set} to obtain a stable solution to \cref{problem:optimal_blocking} for a general semi-Markovian causal graph, $\mathcal{G}$ given in \cref{fig:final_implementation1G}.
\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Z7) [below of=Y] {\scriptsize $V_7$};
  \node[main node] (Z8) [below right of=Z2] {\scriptsize $V_8$};
  \node[main node] (Z9) [above left of=X] {\scriptsize $V_9$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Y) to node {} (Z7);
  \draw[->] (Z1) to node {} (Y);
  \draw[->, bend right] (Z1) to node {} (X);
  \draw[->, bend right] (Z3) to node {} (X);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->, bend left] (Z8) to node {} (Z7);
  \draw[->] (Z9) to node {} (X);
  \draw[->] (Z6) to node {} (Y);
  \draw[->, bend left] (Z2) to node {} (Z7);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Original Graph $\mathcal{G}$.} \label{fig:final_implementation1G}
\end{figure}

\begin{figure}[h!]
\centering
\begin{minipage}{0.42\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Z7) [below of=Y] {\scriptsize $V_7$};
  \node[main node] (Z8) [below right of=Z2] {\scriptsize $V_8$};
  \node[main node] (Z9) [above left of=X] {\scriptsize $V_9$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Y) to node {} (Z7);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z6) to node {} (Y);
  \draw[->, bend left] (Z8) to node {} (Z7);
  \draw[->, bend left] (Z2) to node {} (Z7);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Graph $\mathcal{G}_{\widetilde{X}}$.} \label{fig:figure8}
\end{minipage}
\begin{minipage}{0.42\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Z6) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Graph $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$.}\label{fig:final_implementation1Gnew}
\end{minipage}
\end{figure}

We first obtain the graph $G_{An_{\widetilde{X}}(Y)}$ as displayed in \cref{fig:final_implementation1Gnew}. We next obtain the $c$-components (following \cref{def:c_component}) of $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$ are $\{X\}, \{V_1,V_5,Y,V_2\}, \{V_3\},\{V_4\}$, and the $c$-component of $Y$ is $\{V_1,V_5,Y,V_2\}$. We next obtain the set of parents of the $c$-component of $Y$ as %$\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\} =
$\{X,V_1,V_2,V_3,V_4,V_5\}$. The set $\mathcal{D}(X) \cap \mathcal{A}(Y)$ is $\{X,Y,V_5,V_6\}$. Finally, we obtain the final set as  $(\{X,V_1,V_2,V_3,V_4,V_5\}\backslash\{X\})\backslash(\{X,Y,V_5,V_6\}\backslash\{X,Y\}) = \{V_1,V_2,V_3,V_4\}$.

==> stable-causal-blocking-arxiv/packages_clear.tex <==
%------ USEFUL PACKAGES START HERE ------
\usepackage{hyperref}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{amsthm}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}{Lemma}
% \newtheorem{claim}{Claim}
%\newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{proposition}{Proposition}
\newtheorem{problem}{Problem}
% \newtheorem{remark}{Remark}
%\usepackage{cite}
%\usepackage{algorithm}
% \usepackage{algpseudocode}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{mathtools}
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclareMathOperator*{\argmax}{arg\,max} 
\DeclareMathOperator*{\argmin}{arg\,min} 

%----packages and options for tikz start here
\usepackage[utf8]{inputenc}
\usepackage{pgfplots}
%\DeclareUnicodeCharacter{2212}{−}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}
%\pgfplotsset{compat=1.15,width=7cm,height=7cm}
%\pgfplotsset{scaled y ticks=false}
%\usepackage{caption}
%\usepackage{subcaption}
%----packages and options for tikz end here
%------ USEFUL PACKAGES END HERE ------

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{caption}
\usepackage{subcaption}
%\usepackage{amsthm}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}[theorem]
%\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{note}{Note}
%\newtheorem{definition}{Definition}
%\newtheorem{assumption}{Assumption}
%\newtheorem{proposition}{Proposition}
%\newtheorem{remark}{Remark}
%\newtheorem{observation}{Observation}
%\usepackage{amsmath}
%\DeclareMathOperator*{\argmax}{arg\,max} 
%\DeclareMathOperator*{\argmin}{arg\,min}  
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usepackage{listings}
\lstset{language=Matlab}
\lstset{breaklines}
\def\munderbar#1{\underline{\sbox\tw@{$#1$}\dp\tw@\z@\box\tw@}}
\lstset{basicstyle=\small, numbers=left, numberstyle=\tiny,stringstyle=\ttfamily,frame=box,commentstyle=\color{blue},showstringspaces=false}
\lstset{extendedchars=false}

\usepackage{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}
\crefname{section}{Section}{sections}
\crefname{problem}{Problem}{problems}
\usepackage{amssymb}

\def\Var{{\textrm{Var}}\,}
\def\E{{\mathbb{E}}\,}
\def\P{{\mathbb{P}}\,}

==> stable-causal-blocking-arxiv/sections-clear/abstract.tex <==
\begin{abstract}
    \textit{Randomized experiments} are often performed to study the causal effects of interest. \textit{Blocking} is a technique to precisely estimate the causal effects when the experimental material is not homogeneous. It involves stratifying the available experimental material based on the covariates causing non-homogeneity and then randomizing the treatment within those strata (known as \textit{blocks}). This eliminates the unwanted effect of the covariates on the causal effects of interest. We investigate the problem of finding a \textit{stable} set of covariates to be used to form blocks, that minimizes the variance of the causal effect estimates. Using the underlying causal graph, we provide an efficient algorithm to obtain such a set for a general \textit{semi-Markovian} causal model.
\end{abstract}


==> stable-causal-blocking-arxiv/sections-clear/abstract_clear.tex <==
\begin{abstract}
    \textit{Randomized experiments} are often performed to study the causal effects of interest. \textit{Blocking} is a technique to precisely estimate the causal effects when the experimental material is not homogeneous. It involves stratifying the available experimental material based on the covariates causing non-homogeneity and then randomizing the treatment within those strata (known as \textit{blocks}). This eliminates the unwanted effect of the covariates on the causal effects of interest. We investigate the problem of finding a \textit{stable} set of covariates to be used to form blocks, that minimizes the variance of the causal effect estimates. Using the underlying causal graph, we provide an efficient algorithm to obtain such a set for a general \textit{semi-Markovian} causal model.
\end{abstract}

\begin{keywords}%
  Causal graphs, randomized experiments, block designs, variance reduction.
\end{keywords}


==> stable-causal-blocking-arxiv/sections-clear/conclusion.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}
We have obtained a statistically optimal blocking set ($\textit{\textbf{Z}}^*$) such that it is the smallest subset of the observed covariates ($Z_1, \cdots, Z_n$) (excluding the forbidden ones) which will account (through blocking) for the maximum possible elimination of variability in response ($Y$). Further perspective on optimality is to prune a statistically optimal blocking set for economic reasons. For instance, suppose that we are restricted to creating blocks using at most $k$ covariates and a statistically optimal blocking set is of cardinality $>k$. One possible way to \textit{optimally} prune a statistically optimal blocking set is by dropping the covariates which are least significant in controlling the variability in response.
Or the question can be what is the minimum number of covariates required to eliminate as much as $(1-\alpha)\times 100 \%$ of the variability eliminated by a statistically optimal blocking set, for some user-defined $0\le\alpha\le1$. The idea is to do constrained optimization, where the constraint is usually a user-defined economic cost restriction.

Hence, we need to have a way to decompose the total variability controlled by a statistically optimal blocking set in terms of its individual elements, i.e., to quantify the contribution of each individual covariate in the optimal blocking set controlling the variability in the response. For the example graph in \cref{fig:figure7}, we have seen that a statistically optimal blocking set is $\textit{\textbf{Z}}^* = \{Z_1,Z_2,Z_3,Z_4\}$. We are interested in further pruning this set due to economic reasons. Note that, $Z_1$ and $Z_2$ are the parents of $Y$ and have direct effect on $Y$ through $Z_1 \rightarrow Y$ and $Z_2 \rightarrow Y$, respectively. $Z_4$ affects $Y$ through either of the routes viz., through $Z_4 \rightarrow Z_2 \rightarrow Y$ when $Z_2$ is unblocked, and through $Z_4 \rightarrow Z_2 \leftrightarrow Y$ when $Z_2$ is blocked. Similarly, $Z_3$ also affects $Y$ one of the two routes.

Suppose it is possible to quantify all the causal effects through the observed variables then we can take the following subgraph of \cref{fig:figure9} the with varying thickness of the edges between observed variables, where the thickness represents the strength of the link.

\begin{figure}[h!]
\centering
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10a}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->] (Z2) to node {} (Y);
  \draw[->,ultra thick] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10b}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->,ultra thick] (Z2) to node {} (Y);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10c}
\end{minipage}
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.2cm,thin,main node/.style={circle,draw,font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (Y)  [] {\tiny $Y$};
  \node[main node] (Z2) [above right of=Y] {\tiny $Z_2$};
  \node[main node] (Z4) [above right of=Z2] {\tiny $Z_4$};
  
  \begin{scope}
  \draw[->,ultra thick] (Z2) to node {} (Y);
  \draw[->,ultra thick] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\subcaption{}\label{fig:figure10d}
\end{minipage}
\caption{Subgraphs of \cref{fig:figure9} involving $\{Z_4,Z_2,Y\}$ with varying link strengths.}
\end{figure}

In \cref{fig:figure10a} both the links are weak, hence we can discard both. In \cref{fig:figure10b} the link $Z_4 \rightarrow Z_2$ is strong but the strength of the effect of $Z_4$ on $Y$ through the path $Z_4 \rightarrow Z_2 \rightarrow Y$ depends on how strong the link $Z_2 \rightarrow Y$ is? It can be seen that in Figure 14(b) the link $Z_2 \rightarrow Y$ is weak which suggest that we can discard $Z_2$ and as long as we don't block $Z_2$ we never open the path $Z_4 \rightarrow Z_2 \rightarrow Y$, and hence we can discard $Z_4$ also. In \cref{fig:figure10c} the link  $Z_2 \rightarrow Y$ is strong which suggest that we should block $Z_2$. Blocking $Z_2$ will open the path the $Z_4 \rightarrow Z_2 \rightarrow Y$ but as the link $Z_3 \rightarrow Z_4$ is weak we can discard $Z_4$. In \cref{fig:figure10d} the link $Z_2 \rightarrow Y$ is strong which suggest that we should block $Z_2$. Blocking $Z_2$ will open the path the $Z_4 \rightarrow Z_2 \rightarrow Y$ and as the link $Z_3 \rightarrow Z_4$ is strong we should block $Z_4$ also.

The discussion can be used to motivate towards how and when further pruning of a statistically optimal blocking set can be done due to economic reasons. But there are several issues as follows.
\begin{enumerate}
\item Quantification of causal effects will require some observational data which may be difficult specifically for the treatment and response variables. Though all the covariates that we need to worry about are all pre-treatment and pre-response which are usually observed.
\item Even with the availability of some observational data for some or all variables, it may be possible that the causal effect is not identifiable.  
\end{enumerate}

In the case of some specific cases of linear models simple linear regression and Wright's rule can be of some help. But making some general statements is very difficult. For instance, the strength of the links $Z_4 \rightarrow Z_2$ and $Z_3 \rightarrow Z_4$ can be assessed by regressing $Z_4$ on $Z_2$, and $Z_3$ on $Z_1$.

In general, an economic restriction may not just be on the number of covariates to block using. As seen in the example in Section \ref{sec:challenges}, the economic cost of blocking depends also on the dimensionality of the covariates. Hence, one possible way to think about the economic cost of a blocking set is the resulting no. of blocks. But, the cost of a blocking set may not just be the no. of blocks. It can also involve how costly each covariate is otherwise. For instance, blocking using gender may be costlier than using age, though gender results in 2 blocks and age result in 4 blocks. Hence, the general definition of the economic cost of a blocking set should account for the resulting no. of blocks and the cost of forming those blocks for different covariates in that blocking set.


{\bf Some text needed}
\begin{definition}
The \textit{economic cost of a blocking set} is defined as a weighted sum of the dimensions of the covariates in it, where weights are their individual costs of forming blocks.
\end{definition} 
Note that, when all the covariates are equally costly and are of the same dimension, the cost of blocking is nothing but its cardinality, the case which we have considered at the beginning of this section.

{\bf Some text needed}
\begin{definition}
The \textit{statistical cost of a blocking set} is defined as the inverse of the amount of variability in the response that it controls for.
\end{definition}
Note that, we haven't completely addressed how to quantify the statistical cost of blocking.

{\bf Some text needed}
\begin{definition} \label{def:optimal_blocking_set}
The smallest subset of the set of observed covariates (excluding some forbidden variables if there are any) is said to be an \textit{optimal blocking set} if it minimizes the statistical cost of blocking among all the subsets of the set of observed covariates (excluding some forbidden variables if there are any), having an economic cost less than or equal to some user-defined threshold.
\end{definition} 

Developing an algorithm to obtain an optimal blocking set defined in Definition \ref{def:optimal_blocking_set} is an open problem that we aim to address in our future work.

==> stable-causal-blocking-arxiv/sections-clear/conclusion_v0.02.tex <==
\section{Conclusion and Future Work} \label{sec:conclusion}
We investigated the problem of finding a stable set of covariates to be used for forming blocks, that minimizes the variance of the causal effect estimates. By leveraging the underlying causal graph, we provided an efficient algorithm to obtain such a set for a general semi-Markovian causal model. 

In the future, we are interested in extending our work towards further pruning the stable causal blocking set obtained in this paper for the reasons of economic cost. If the experimenter has a constraint on the cardinality (size) of the blocking set due to budget limitations, i.e. $|\mathcal{Z}| \le k_1$ where $k_1$ is specified by the experimenter. Furthermore, if blocking variables have different economic costs associated with them, for example, getting data on cholesterol level may be costlier (or difficult) as compared to the age of the patient, then we can introduce a knapsack budget constraint. Let $e(Z)$ be the cost associated with $Z\in \mathcal{Z}$ then the knapsack constraint would be $\sum_{Z\in\mathcal{Z}}e(Z) \le k_2$ where $k_2$ is specified by the experimenter. We are interested in solving the problem of finding stable solutions to \cref{problem:optimal_blocking} with additional cardinality or knapsack constraint on the feasible solutions. Furthermore, we are interested in extending our work for the cases when the treatment and response variables are sets of variables. For the future direction to use the proposed algorithm for different real-world applications, refer to \cref{app:future}. \\

%\acks{The author thanks the anonymous reviewers, Dr. Christopher J. Quinn from Iowa State University, and Dr. Vaneet Aggarwal from Purdue University, for their valuable suggestions.}

==> stable-causal-blocking-arxiv/sections-clear/experiments.tex <==
\section{Experimental Evaluations} \label{sec:experiments}

In this section, we provide experimental evaluations to compare our method with other choices of sets of covariates to create blocks. For the causal graph, $\mathcal{G}$ provided in \cref{fig:final_implementation1G}, we are interested in studying the causal effect of Drug ($X$) on Blood-Pressure ($Y$). 

We considered a simple setting where all variables under consideration are binary variables taking values in \{0,1\}. We used a simple joint probability distribution that factorizes according to the given causal graph. We then performed simulated randomized experiments for different choices of sets of covariates to create blocks. The estimated causal effect and the variability in the response for different choices of blocking sets are provided in \cref{tab:causal_effect}. We observe that the variability in the response is the smallest for the choice of covariates obtained using the algorithm proposed in this paper. For details of the experimental evaluations, refer to \cref{app:exp_details}.

\begin{table*}[t] 
    \centering 
    \caption{Causal effect estimate and variability in the response.}  \label{tab:causal_effect}
	\begin{tabular}{l r r}
		\hline \hline
		  Blocking set & Causal effect & Variance \\
            \hline
            $\phi$, i.e. no blocking & 0.6910 & 0.2126 \\
            \{Food Habits\} & 0.6950 & 0.2098 \\
            \{Food Habits, Alcohol\} & 0.6960 & 0.2028 \\    
            \{Food Habits, Alcohol, Cholesterol\} & 0.6760 & 0.2001 \\     
            \{Food Habits, Alcohol, Cholesterol, Age\} & 0.7150 & 0.1754\\
	    \hline
	    \hline
	\end{tabular}
\end{table*}

==> stable-causal-blocking-arxiv/sections-clear/extra.tex <==
There can be two types of causal effect that one might be interested in estimating, viz.,
\begin{enumerate}
    \item individual causal effect for the $i$th unit, i.e. the causal effect of $X_i$ on $Y_i$, and
    \item overall causal effect of $X$ on $Y$ 
\end{enumerate}

Let $Y_i$ be the response for the $i$th unit. Define the response for the $i$th unit when it receives the treatment as
\begin{align}
Y_{1i} &: = Y_i \text{ when } X_i=1.
\end{align}
Define the response for the $i$th unit when it does not receive the treatment as
\begin{align}
Y_{0i} &:= Y_i \text{ when } X_i=0.
\end{align}
\citet{rosenbaum1983central} termed $Y_{1i}$ and $Y_{0i}$ as \textit{potential outcomes} for the $i$th unit when it receives the treatment and when it is under control, respectively. 

For the $i$th unit, we can define the causal effect of the treatment as the difference between the potential outcomes under treatment and control, i.e., $Y_{1i}-Y_{0i}$. However, individual treatment effects cannot be calculated as we only observe $X_i$ and $Y_i = X_iY_{1i} + (1-X_i)Y_{0i}$ \citep{holland1986statistics}, which is due to the fact that we don't assign treatment to all the units rather we randomize. Because of this missing data problem, attention has been focused on some parameters which can summarize the causal effect, usually in terms of expectations. Following \citep{heckman1992randomization}, \citep{clements1994making}, and \citep{heckman1995assessing}, we define the \textit{effect of treatment} (ET) in the population as
\begin{align}
\beta = E(Y_{1}-Y_{0}), \text{ and}
\intertext{the \textit{effect of treatment on treated} (ETT) in the population as}
\gamma = E((Y_{1}-Y_{0})|X=1).
\end{align}

We focus on estimation of $\beta = E(Y_{1}-Y_{0})$. We introduce the following notations.
\begin{align*}
    I_1 &= \{i:X_i=1\}, \ n_1 = |I_1|,\\
    I_0 &= \{i:X_i=0\}, \ n_0 = |I_0|.
\end{align*}

The natural non-parametric estimate of this expectation is the corresponding sample average, and is given as
\begin{align}
\hat{\beta} &= \frac{1}{n_1}\sum_{i:X_i=1}Y_{1i}-\frac{1}{n_0}\sum_{i:X_i=0}Y_{0i} \nonumber \\ 
&:= \bar{Y}_1 - \bar{Y}_0. \label{def:sample_mean}
\end{align}

$E(\hat{\beta}) = \beta$, i.e., $\hat{\beta}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}$ (normalized for sample size) is given as follows.
\begin{align}
    V(\hat{\beta}) = 
      E_Z\bigg(\frac{V(Y_1|Z)}{P(X=1|Z)} &+ \frac{V(Y_0|Z)}{P(X=0|Z)} \nonumber \\ &\text{} + (\beta(Z)-\beta)^2 \bigg) \label{eq:var_under_no_blocking}
\end{align}

% \begin{align}
%     V(\hat{\beta}) & = 
%     \begin{cases}
%       E_Z\left(\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  + (\beta(Z)-\beta)^2 \right), & \text{under non-homogeneity},\\
%       \frac{V(Y_1)}{P(X=1)} + \frac{V(Y_0)}{P(X=0)}, &  \text{under homogeneity}. \tag{2} \label{eq:var_under_no_blocking}
%     \end{cases}
% \end{align}

Prior works \citep{} suggest to do blocking in the situation when the experimental units are not homogeneous. Let us see how does the estimator $\hat{\beta}$ defined in Equation \ref{def:sample_mean} should be updated, under blocking using covariates in $Z$. Following Theorem \ref{} of \citep{petersen2006estimation}, we have
\begin{align}
\beta &= E(Y_{1}-Y_{0}) = E_Z\left(E((Y_{1}-Y_{0})|Z)\right), \nonumber\\ 
&= E_Z\left(E(Y_{1}|Z)-E(Y_{0}|Z)\right) \nonumber \\ 
&= \sum_{Z=z}\left(E(Y_{1}|Z=z)-E(Y_{0}|Z=z)\right)P(Z=z).
\end{align}
Hence, we can define an estimator of $\beta$ under blocking using covariates in $Z$, as follows.
\begin{align}
\hat{\beta}_Z & = \sum_{Z=z}\left(\hat{E}(Y_{1}|Z=z)-\hat{E}(Y_{0}|Z=z)\right)\hat{P}(Z=z), \nonumber \\
&= \sum_{Z=z}\left((\bar{Y_{1}}|Z=z)-(\bar{Y_{0}}|Z=z)\right)\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)},
\end{align}
where $\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)}$ is the proportion of units in the block formed with characteristics $Z=z$.

Suppose there are no units in one or more blocks, i.e., $\frac{1}{n}\sum_{i=1}^{n}{I(Z_i=z)} = 0$ for some $z$, then the overall average treatment effect can be estimated but the $z$-specific causal effect cannot be estimated. Hence, it is desirable to have units in every block. This also rules out the argument against randomized block experiments that matching of units can be done post a completely randomized experiment based on the covariates, as it is possible that there are no units corresponding to a particular covariate combination.

$E(\hat{\beta}_Z) = \beta$, i.e., $\hat{\beta}_Z$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}_Z$ (normalized for sample size) is given as follows.
\begin{align}
    V(\hat{\beta}_Z) = E_Z\bigg(&\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  \nonumber \\  &\text{ } + \big(\sum_Z\beta(Z)\hat{P}(Z) - \beta \big)^2 \bigg) \label{eq:var_under_blocking}
\end{align}
% \begin{align}
%     V(\hat{\beta}_Z) & = 
%     \begin{cases}
%       E_Z\left(\frac{V(Y_1|Z)}{P(X=1|Z)} + \frac{V(Y_0|Z)}{P(X=0|Z)}  + \left(\sum_Z\beta(Z)\hat{P}(Z) - \beta \right)^2 \right), & \text{non-homogeneity},\\
%       \frac{V(Y_1)}{P(X=1)} + \frac{V(Y_0)}{P(X=0)}, &  \text{homogeneity}.
%     \end{cases} \tag{4} \label{eq:var_under_blocking}
% \end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gain in Precision due to Blocking}
Consider a simple setting where $X$ is an indicator random variable defined as
\begin{equation}
X = 
\begin{cases} 
    1, & \text{if the treatment is applied}, \\
    0, & \text{otherwise,}
\end{cases}
\end{equation}
and $Y$ is real-valued random variable.

Let there be $n$ experimental units available to study the causal effect of $X$ on $Y$ by performing a randomized experiment. Let $\mathcal{Z}$ denote the set of covariates that vary across the experimental units. 

We want to demonstrate the gain in precision due to blocking. Hence, we first ignore these covariates and perform a CRD as follows. We randomize $X$ over the available experimental units, i.e. randomly assign a unit to either have the treatment ($X=1$) or not ($X=0$), and then observe the response. Let $(X_i,Y_i)$ denote the treatment and response pair for the $i$th experimental unit. %As different units are identical and we have randomized the treatment, $X_i$ and $Y_i$ are nothing but i.i.d. copies of $X$ and $Y$, respectively. In other words, $\{(X_i,Y_i): i=1,\dots,n\}$ is a random sample from ($X,Y$). 
Define $I_x:=\{i:X_i=x\}$ and $n_x:=|I_x|$. 

%denote the set of indices of units where the value of treatment, and $I_1:=\{i:X_i=0\}$ denote the set of indices of units where the treatment is not applied. Further, define $n_1:=|I_1|$ and $n_0:=|I_0|$.

We are interested in estimating $\mathbb{E}(Y|do(X))$. For simplicity, define $Y(x) := Y|do(X=x)$. For our simple setting, we have only two possibilities of the that conditional expectation, viz. $\mathbb{E}(Y(1))$ and $\mathbb{E}(Y(0))$.  Similar to \citep{heckman1992randomization}, \citep{clements1994making}, and \citep{heckman1995assessing}, we define the \textit{effect of treatment} (ET) in the population as
\begin{align}
\beta := \E(Y(1)) - \E(Y(0)). \label{eq:beta}
\end{align}
A natural non-parametric estimator of $\E(Y(x))$ is the corresponding sample average, given as
\begin{align}
\bar{Y}(x) &:= \frac{1}{n_x}\sum_{i\in I_x}Y_{i}.
\end{align}
Hence, we can estimate $\beta$ as
\begin{align}
\hat{\beta} &= \bar{Y}(1) - \bar{Y}(0)
\end{align}

It can be shown that $\mathbb{E}(\hat{\beta}) = \beta$, i.e., $\hat{\beta}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{\P(X=1|\mathcal{Z})} + \frac{\Var(Y(0)|\mathcal{Z})}{\P(X=0|\mathcal{Z})} \right) \nonumber \\ 
      \text{} + \mathbb{E}_\mathcal{Z}\left((\beta(\mathcal{Z})-\beta)^2 \right), \label{eq:var_under_no_blocking}
\end{align}
where $\beta(\mathcal{Z}):= \E(Y(1)|\mathcal{Z}) - \E(Y(0)|\mathcal{Z})$ is the $\mathcal{Z}$-specific causal effect. For proofs of unbaisedness and variance of $\hat{\beta}$, see Appendix.

We now perform an RBD as follows. We first stratify the experimental units such that units with each stratum (known as block) are identical, i.e. the covariates in $\mathcal{Z}$ remain same with a block. We next randomize $X$ over the experimental units within each block, and then observe the response. Let $(X_i,Y_i,\mathcal{Z}_i)$ denote the treatment, response, and covariates triplet for the $i$th experimental unit. Define $I_{x,z}:=\{i:X_i=x,\mathcal{Z}_i = z\}$ and $n_{x,z}:=|I_{x,z}|$. 

Note that ET defined in \eqref{eq:beta} can be re-written as \citep{petersen2006estimation}
\begin{align}
    \beta &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}\right) - \E_\mathcal{Z}\left(\E(Y(0) | \mathcal{Z}\right), \nonumber\\
    &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}) - \E(Y(0) | \mathcal{Z})\right), \nonumber\\
    &= \sum_{\mathcal{Z} = z} \left(\E(Y(1) | \mathcal{Z}=z) - \E(Y(0) | \mathcal{Z}=z) \right) \P(\mathcal{Z}=z) \label{eq:beta_z}
\end{align}
A natural non-parametric estimator of $\E(Y(x)|\mathcal{Z}=z)$ is the corresponding sample average, given as
\begin{align}
    \bar{Y}(x)|(\mathcal{Z}=z) &:= \frac{1}{n_{x,z}}\sum_{i\in I_{x,z}} Y_i
\end{align}
$\P(\mathcal{Z}=z)$ can be estimates as
\begin{align}
    \hat{\P}(\mathcal{Z}=z) &:= \frac{n_{x,z}}{n}
\end{align}
Hence, we can estimate $\beta$ as
\begin{align}
\hat{\beta}_\mathcal{Z} &= \frac{1}{n}\sum_{\mathcal{Z} = z} n_{x,z} \left(\bar{Y}(1) | (\mathcal{Z}=z) - \bar{Y}(0) | (\mathcal{Z}=z) \right)
\end{align}
It can be shown that $\mathbb{E}(\hat{\beta}_\mathcal{Z}) = \beta$, i.e., $\hat{\beta}_\mathcal{Z}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}_\mathcal{Z}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}_\mathcal{Z}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{\P(X=1|\mathcal{Z})} + \frac{\Var(Y(0)|\mathcal{Z})}{\P(X=0|\mathcal{Z})} \right) \nonumber \\ 
      \text{} + \mathbb{E}_\mathcal{Z} \left(\left(\sum_{\mathcal{Z}=z}\beta(\mathcal{Z}=z)\hat{\P}(\mathcal{Z}=z) - \beta \right)^2\right), \label{eq:var_under_blocking}
\end{align}
For proofs of unbaisedness and variance of $\hat{\beta}_\mathcal{Z}$, see Appendix.

By comparing \eqref{eq:var_under_no_blocking} and \eqref{eq:var_under_blocking}, we observe that $\Var(\hat{\beta}_\mathcal{Z}) \le \Var(\hat{\beta})$, i.e. blocking improves the precision of the estimate of the population average causal effect, $\beta$.

%Another example to demonstrate the gain in precision due to blocking is as follows. Suppose there are $k$ treatments and $b$ blocks, then the response can be defined as a linear equation: $y_{ij} = \mu + \tau_i + b_j + \epsilon_{ij}$, where $\mu$ is the general mean effect, $\tau_i$ is the effect due to the the $i$th treatment, $b_j$ is the effect due to the $j$th block, and $\epsilon_{ij}$ is the noise or the experimental error. Clearly, in the absence of $b_j$, error is higher as compared to the case when $b_j$ is there.

%If the experimental units are identical then $\hat{\beta}_\mathcal{Z} = \hat{\beta}$. 

%\textbf{Remark.} Suppose there are no units in one or more blocks, i.e., $n_{x,z} = 0$ for some $z$, then the overall average treatment effect can be estimated but the $z$-specific causal effect cannot be estimated. Hence, it is desirable to have units in every block. This also rules out the argument against randomized block experiments that matching of units can be done post a completely randomized experiment based on the covariates, as it is possible that there are no units corresponding to a particular covariate combination.

%\subsection{Gain in Precision under Blocking} We have seen that blocking improves the precision of the estimates. Sometimes, the interest is to study the causal effects from the observational data, possibility because carrying out a randomized experiment is either economically or ethically infeasible. An approach similar to blocking (in randomized experiments) called \textit{matching} is used to study the causal effects from the observational data, where grouping of units is done on covariates after getting the observational data. There covariate adjustment is done to reduce the confounding bias. For instance, \citep{rosenbaum1983central} provided a way to create blocks by matching the observation on propensity score, which is a famously termed as \textit{propensity score matching} (PSM). General concerns with matching have been raised by \citet{pearl2009causality}, who has argued that hidden bias may actually increase because matching on observed variables may unleash bias due to dormant unobserved confounders. Similarly, \citet{pearl2009causality} has argued that bias reduction can only be assured (asymptotically) by modeling the qualitative causal relationships between treatment, outcome, observed and unobserved covariates. Confounding occurs when the experimenter is unable to control for alternative, non-causal explanations for an observed relationship between independent and dependent variables. Such control should satisfy the \textit{back-door criterion} \citep{pearl2009causality}.



\begin{figure}[th]
\centering
\begin{minipage}{.49\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \end{scope}
\end{tikzpicture}
\caption{Example Markovian model.} \label{fig:figure1}
\end{minipage}
\begin{minipage}{.49\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize  $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \end{scope}
\end{tikzpicture}
\caption{Example semi-Markovian model with latent variables involving only covariates.} \label{fig:figure2}
\end{minipage}
\end{figure}

==> stable-causal-blocking-arxiv/sections-clear/introduction.tex <==
\section{Introduction}

\subsection{Motivation}
Studying the \textit{causal} effect of some variable(s) on the other variable(s) is of common interest in social sciences, computer science, and statistics. However, a mistake that people usually make is, confusing the causal effect with an \textit{associational} effect. For instance, if high levels of bad cholesterol and presence of a heart disease are observed at the same time, it does not mean that the heart disease is caused by the high levels of bad cholesterol. The question is then how do we get to know if at all a variable causes the other? If the answer is yes, then what is the direction (positive or negative) and what is the magnitude, of the causal effect? \cite{fisher1992statistical} provided the framework of \textit{randomized experiments} to study the causal effect, where the variable whose causal effect is to be studied (known as \textit{treatment} or cause), is randomized over the available experimental material like humans, rats, agricultural plots etc. and changes in the variable on which the causal effect is to be studied  (known as \textit{response} or effect), are recorded. A statistical comparison of values of the response with or without the treatment can therefore be done to study the existence, direction and magnitude of the cause-effect relationship of interest.

Randomized experiments work on three basic principles, viz., \textit{randomization}, \textit{replication}, and \textit{local control}. Randomization states that the assignment of the treatment has to be random, replication states the treatment should be given to multiple but homogeneous units, i.e., there are multiple observations of the effect variable for both with and without the treatment. Hence, as long as the entire experimental material is homogeneous (for instance, the fertility of all the agricultural plots is same, the responsiveness of all the humans is same for the drug, etc.), then a `good' randomized experiment can be carried out using the first two principles, viz., randomization and replication, which gives rise to  \textit{completely randomized design} (CRD). However, when the entire experimental material is not homogeneous, i.e., some attributes of experimental units (known as \textit{covariates}) differ from each other, then the causal effect may get influenced by the covariates causing non-homogeneity like fertility, responsiveness, etc. The remedy to this problem is the third principle of randomized experiments, i.e., local control (also known as \textit{blocking}), which states to stratify the entire experimental material based on that covariate(s) causing non-homogeneity, and then randomize the treatment within those strata to eliminate the effect of the covariates. These strata are called \textit{blocks}, and this third principle along with the first two give rise to  \textit{randomized block design} (RBD). Blocking tries to control/eliminate the variability in the response attributed through the covariates and leads to a more \textit{precise} estimation of the caual effect of interest. %Precision is defined as inverse of the variability which measures how much the response would have varied if the sample would have changed. In the context of estimating the causal effects, precision is  the inverse of the variance of the estimate of the causal effect. 

In this paper, we focus on the problem of deciding which covariates to use for creating the blocks while performing a randomized experiment. We consider a non-parametric setting and assume that we have access to the underlying structural causal model \cite{pearl2009causality}. We provide a graphical criterion to obtain a statistically optimal set of covariates to use for creating the blocks for a general semi-Markovian causal graph.

\subsection{Literature Review}
Statistics literature \cite{yates1935complex}, \cite{kempthorne1952design}, \cite{kempthorne1955randomization}, \cite{cochran1948experimental} presents profound discussions on relative efficiency (ratio of the variances of causal effects) of RBD over CRD. It can be seen that in general, RBD is always more or at least as efficient as CRD. Hence, the natural question is how do we do blocking in an intelligent manner such that maximum gain in precision can be attained, i.e., variability in the response due to the covariates, can be controlled to a maximum possible extent? More specifically, we are interested in knowing which all covariates should be used to create blocks? Intuitively, we can say that we need not take the ones into consideration which remain constant in the population. But, among the ones which vary, can we choose some over the other, using some criterion? 

Most of the blocking schemes discussed in the literature discuss about creating blocks by grouping the experimental units which are close to each other based on some attributes. For instance, \textit{threshold blocking} \cite{higgins2016improving}.

The question that we are interested in answering is, can we decide which covariates to use for creating blocks using the causal structure (diagram) of the all the variables, viz., treatment, response and covariates (observed and unobserved), provided the causal structure is given?

\subsection{Contribution}
The main contributions of this paper can be summarized as follows.
\begin{enumerate}
    \item We formalize the problem of obtaining a statistically optimal set of covariates to be used to create blocks in randomized experiments under a non-parametric setting.
    \item We provide a graphical test to obtain such a set for a general semi-Markovian causal model. 
    %\item We also propose and provide ideas towards solving a more general problem of obtaining an optimal blocking set that considers both the statistical and economic costs of blocking.
\end{enumerate}

\subsection{Organization}
The rest of the paper is organized as follows. \Cref{sec:prob_formulation} provides some background and formulates the problem of interest. \Cref{sec:methodology} first discusses some key observations and motivating examples, and then provides the main results. \Cref{sec:conclusion} concludes the paper and provides future directions.

==> stable-causal-blocking-arxiv/sections-clear/introduction_v0.02.tex <==
\section{Introduction}

\subsection{Motivation} \label{sec:motivation}
Studying the \textit{causal} effect of some variable(s) on the other variable(s) is of common interest in social sciences, computer science, and statistics. However, a mistake that people usually make is confusing the causal effect with an \textit{associational} effect. For instance, if high levels of bad cholesterol and the presence of heart disease are observed at the same time, it does not mean that the heart disease is caused by high levels of bad cholesterol. The question is then how do we get to know if one variable causes the other? If the answer is yes, then what is the direction (positive or negative) and what is the magnitude, of the causal effect? \citet{fisher1926arrangement} provided the framework of \textit{randomized experiments} to study the causal effect, where the variable whose causal effect is to be studied (known as \textit{treatment} or cause), is randomized over the available experimental units (like humans, rats, agricultural plots, etc.) and changes in the variable on which the causal effect is to be studied  (known as \textit{response} or effect), are recorded. A statistical comparison of values of the response with or without the treatment can therefore be done to study the existence, direction, and magnitude of the cause-effect relationship of interest.

Randomized experiments work on three basic principles, viz., \textit{randomization}, \textit{replication}, and \textit{local control} \citep{fisher1926arrangement}. Randomization states that the assignment of the treatment has to be random, and replication states the treatment should be given to multiple but homogeneous units, i.e., there are multiple observations of the effect variable for both with and without the treatment. Therefore, as long as the available experimental units are homogeneous (for instance, the fertility of all the agricultural plots is the same, the responsiveness of all the humans is the same for the drug, etc.), then a `good' randomized experiment can be carried out using the first two principles, viz., randomization and replication, which gives rise to  \textit{completely randomized design} (CRD). However, when the available experimental units are not homogeneous, i.e., some attributes of experimental units (known as \textit{covariates}) differ from each other, then the causal effect may get influenced by the covariates causing non-homogeneity (like fertility, responsiveness, etc). The remedy to this problem is the third principle of randomized experiments, i.e., local control (also known as \textit{blocking}), which states to stratify the available experimental units based on that covariate(s) causing non-homogeneity, and then randomize the treatment within those strata to eliminate the effect of the covariates. These strata are called \textit{blocks}, and this third principle along with the first two gives rise to  \textit{randomized block design} (RBD). %Blocking tries to control/eliminate the variability in the response attributed through the covariates and leads to a reduction in the variance of the estimate of the causal effect of interest.
Blocking tries to control/eliminate the variability in the response attributed through the covariates and leads to a more \textit{precise} estimation of the causal effect of interest. Precision is defined as the inverse of the variance of the estimate of the causal effect of interest.

In this paper, we focus on the problem of deciding which covariates to be used for forming the blocks while performing a randomized experiment. We consider a non-parametric setting and assume that we have access to the underlying causal structure \citep{pearl2009causality}. We provide an efficient algorithm to obtain a \textit{stable} set of covariates to be used to form blocks for a general semi-Markovian causal model. The term stable refers to the idea of finding and excluding the covariates that one should never use to create blocks. The notion and the method of achieving this stability are discussed in \cref{sec:stable_blocking}.

\subsection{Literature Review}
Statistics literature \citep{yates1935complex, kempthorne1952design, kempthorne1955randomization, cochran1948experimental} presents profound discussions on relative efficiency (ratio of the variances of causal effects) of RBD over CRD. It can be seen that in general, RBD is always more or at least as efficient as CRD. Therefore, the natural question is how do we do blocking in an intelligent manner such that maximum gain in precision can be attained? More specifically, we are interested in answering the following question. Can we decide which covariates to be used for forming blocks using the causal structure (diagram) of all the variables, viz., treatment, response, and covariates (observed and unobserved) provided the causal structure is given? 

In the past, efforts have been made to address the problem of efficient adjustments in causal graphical models under static interventions \citep{henckel2019graphical, rotnitzky2020efficient} and under dynamic interventions \citep{10.1093/biomet/asab018}. In contrast to these, we provide an efficient algorithm to obtain the set of covariates to be used for forming blocks for a general semi-Markovian causal model. %However, they do not provide a general algorithm to address the problem for a general causal graph. In contrast, we provide an efficient algorithm to obtain the set of covariates to be used for forming blocks for a general semi-Markovian causal model. 
citet{cinelli2020crash} provided a good discussion on good and bad controls for different causal graphs and emphasized the importance of good adjustments in causal estimation. Some other partially related works include \citep{kallus2018optimal} which discusses the problem of experimental design in terms of variance reduction and describes the functional assumptions placed on the potential outcome by blocking, \citep{harshaw2019balancing} which shows that discrepancy minimization (difference in means between treatment and control covariate groups) implicitly performs ridge regression and \citep{li2019rerandomization} talks about re-randomization and regression adjustment.

In this paper, we focus on deciding what covariates should form the basis of forming blocks. However, a problem that follows our problem is, how to efficiently form blocks by grouping the experimental units which are close to each other based on the chosen covariates. \citet{moore2012multivariate,higgins2016improving} focus on the latter problem.

\subsection{Contribution}
In this paper, we formalize the problem of finding a \textit{stable} set of covariates to be used to form blocks, that minimizes the variance of the causal effect estimates. We leverage the underlying causal graph and provide an efficient algorithm to obtain such a set for a general \textit{semi-Markovian} causal model.

\subsection{Organization}
The rest of the paper is organized as follows. \Cref{sec:prob_formulation} provides some background and formulates the problem of interest. \Cref{sec:methodology} discusses our methodology that includes motivating examples, key observations, important lemmas, main results, and the final algorithm. \Cref{sec:experiments} provide experimental evaluations, and \Cref{sec:conclusion} concludes the paper and provides future directions.

==> stable-causal-blocking-arxiv/sections-clear/methodology.tex <==
\section{Methodology} \label{sec:methodology}
In this section, we develop a methodology to find a solution to \cref{problem:optimal_blocking}. We first examine $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$ to obviate some edges and nodes from the causal graph, $\mathcal{G}$. We next discuss some motivating examples and make key observations that lead to several lemmas for our main result. In the end, we provide our main result and develop an efficient algorithm for solving \cref{problem:optimal_blocking}.

\subsection{Examining $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$}
In \cref{problem:optimal_blocking}, our interest is to minimize $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}\subseteq \mathcal{C}$. $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ through the causal relationships from $\mathcal{Z}$ to $Y$, and from $\mathcal{Z}$ to $X$. Note that, $X$ is the treatment on which we are performing the intervention, i.e.,  we set the levels/values of $X$. This is equivalent to saying that $X$ is no longer affected by the rest of the variables. Therefore, $\mathcal{Z}$ also cannot affect $X$ when an intervention is performed on $X$. %instead its value is decided/set during the experiment. %In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all arrows coming into $X$. 
Therefore, $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from $\mathcal{Z}$ to $Y$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}$ to $Y$ gives a solution to \ref{problem:optimal_blocking}.

Denote the subgraph of $\mathcal{G}$ where all edges coming into $X$ were deleted as $\mathcal{G}_{\widetilde{X}}$.
\begin{lemma} \label{lemma:Gxbar}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}_{\widetilde{X}}$.
\end{lemma}
\begin{proof}
The proof follows from the fact that when an intervention is performed on $X$ then it is no longer affected by the rest of the variables. In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all edges coming into $X$. 
\end{proof}

\begin{definition}
$\mathcal{S},\mathcal{T}\subseteq \mathcal{C}$ are called equivalent sets (denoted as $\mathcal{S} \equiv \mathcal{T}$), if  $\Var(\hat{\P}_\mathcal{S}(Y|do(X))) = \Var(\hat{\P}_\mathcal{T}(Y|do(X)))$.
\end{definition}

\begin{lemma} \label{lemma:D0}
If $\mathcal{F}$ is the set of all covariates that do not have causal paths to $Y$, then $\mathcal{C}$ and $\mathcal{C}\backslash \mathcal{F}$ are equivalent sets.
\end{lemma}
\begin{proof}
The proof follows from the fact that a set of covariates can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from itself to $Y$.
\end{proof}
Following \cref{lemma:Gxbar}, we restrict ourselves to the subgraph $\mathcal{G}_{\widetilde{X}}$. Following \cref{lemma:D0}, we further delete the covariates that do not have any causal paths to $Y$. Denote this new subgraph as $\mathcal{G}'_{\widetilde{X}}$ and $\mathcal{C}'=\mathcal{C}\backslash\mathcal{F}$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}'$ to $Y$ in $\mathcal{G}'_{\widetilde{X}}$ gives a solution to \ref{problem:optimal_blocking}.

%As discussed earlier, we are interested in performing a randomized experiment to study the causal effect of interest $X\rightarrow Y$ where we are randomizing the treatment $(X)$. In terms of the causal graph, randomizing $X$ is the same as making interventions to set levels/values of $X$. This means that $X$ is not affected by any variable in the graph, instead, its value is decided/set during the experiment. Therefore, we can \textit{ignore all the arrows coming into $X$} and work with the subgraph of $G$ where all arrows coming into $X$ are ignored. We denote such subgraph as $G_{\widetilde{X}}$. Therefore, for the examples, we work with causal graphs with no arrows coming to $X$.

\subsection{Motivating Examples and Key Observations}

All causal graphs in \cref{fig:markovian_model,fig:semi_markovian_model_C,fig:semi_markovian_model_Y,fig:semi_markovian_model_des,fig:semi_markovian_model_postx} represent represent $\mathcal{G}'_{\widetilde{X}}$. Denote the set of parents of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{P}(W)$.

\textbf{Note.} In all the graphs provided in this paper, a bi-directed edge between any two observed variables is same as those two variables having one or more unobserved ancestors. For example $V_3 \xdashleftrightarrow V_4$.

\textbf{Example 1.} For \cref{fig:markovian_model,fig:semi_markovian_model_C}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. Therefore, $\mathcal{Z}^* = \mathcal{P}(Y)\backslash\{X\}$.
\begin{figure}[th]
\centering
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \end{scope}
\end{tikzpicture}
\caption{Example Markovian model (no latent structures).} \label{fig:markovian_model}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize  $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \end{scope}
\end{tikzpicture}
\caption{Example semi-Markovian model with latent variables involving only $\mathcal{C}'$.} \label{fig:semi_markovian_model_C}
\end{minipage}
\end{figure}

\textbf{Example 2.} For \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is not sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. In \cref{fig:semi_markovian_model_Ya}, the reason is that blocking using $V_2$ opens the path $V_4 \rightarrow V_2 \leftarrow Y$ for $V_4$ to cause variability in $Y$. In \cref{fig:semi_markovian_model_Yb}, the reason is that the latent structure $Y \leftrightarrow V_4$ enables $V_4$ to cause $Y$ even when the path $V_4\rightarrow V_2\rightarrow Y$ is blocked. For both \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{Z}^*=(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$.
\begin{figure}[thb]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Ya}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Yb}
\end{minipage}\hspace{.5cm}
\caption{Example semi-Markovian model with latent variables involving $\mathcal{C}'$ and $Y$.}\label{fig:semi_markovian_model_Y}
\end{figure}

\textbf{Example 3.} For \cref{fig:semi_markovian_model_des}, despite $Y$ having descendants, $(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. This is because descendants of $Y$ can never be a cause of variability in $Y$. In \cref{fig:semi_markovian_model_desa,fig:semi_markovian_model_desb}, $V_5$ (a descendant of $Y$) cannot cause $Y$ through the edge $Y \rightarrow V_5$. Moreover, $V_4$ (an ancestor of $Y$) cannot cause $Y$ through $V_5$ because $V_5$ is a collider on the path $V_4\rightarrow V_5 \leftarrow Y$.

\begin{figure}[th]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[->, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desa}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desb}
\end{minipage}
\caption{Example Semi-Markovian Models with latent variables involving $\mathcal{C}'$ and $Y$, and $Y$ having descendants.}\label{fig:semi_markovian_model_des}
\end{figure}

Denote the set of ancestors (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{A}(W)$. Denote the subgraph of $\mathcal{G}'_{\widetilde{X}}$ restricted to $\mathcal{A}(Y)$ as $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Based on the insights from Examples 1 to 3, we write the following lemma.
\begin{lemma}\label{lemma:GxbarA}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$.
\end{lemma}

\begin{proof}
The proof follows from the fact that the descendants of a node can never be its cause even in the presence of latent structures.
\end{proof}

\subsection{Solution to Problem \ref{problem:optimal_blocking}}

We now combine the insights from \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA} to provide a solution to \cref{problem:optimal_blocking}.

\begin{theorem} \label{theorem:sol_to_optimal_blocking}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ is a solution to \cref{problem:optimal_blocking}.
\end{theorem}
\begin{proof}
The proof follows from the fact that $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. %following \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA}.
\end{proof}

\cref{theorem:sol_to_optimal_blocking} provides a sufficient condition for a set $\mathcal{Z}$ to be a solution to \cref{problem:optimal_blocking}. We next provide a method to construct a set $\mathcal{Z}$ that satisfies this sufficient condition.

Let a path composed entirely of bi-directed edges be called a \textit{bi-directed path}.
\begin{definition}\label{def:c_component} \citep{tian2002general}. 
For a graph $\mathcal{G}$, the set of observed variables $\mathcal{V}$, can be \textit{partitioned} into disjoint groups by assigning two variables to the same group if and only if they are connected by a bi-directed path. Assume that $V$ is therefore partitioned into $k$ groups $\mathcal{S}_1, \dots, \mathcal{S}_k$. We will call each $\mathcal{S}_j; j=1, \dots, k,$ a \textit{$c$-component} of $V$ in $\mathcal{G}$ or a $c$-component (abbreviating confounded component) of $\mathcal{G}$. The $\mathcal{S}_j$ such that $W\in S_j$ is called the \textit{$c$-component of $W$} in $\mathcal{G}$ and is denoted as $C_{W,\mathcal{G}}$. As $\{\mathcal{S}_1, \dots, \mathcal{S}_k\}$ is a partition of $\mathcal{V}$, $c$-component of a variable always exists and is unique.
\end{definition}

In Example 2, we observed that due to the presence of latent structures involving $Y$, $\mathcal{P}(Y)$ was not sufficient to block all causal paths from $\mathcal{C}'$ to $Y$. However the parents of $c$-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ would be sufficient for that purpose. 

\begin{theorem} \label{theorem:sol_to_optimal_blocking_construction}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ is  the set of parents of c-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ excluding $X$ denoted as $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$.
\end{theorem} 
\begin{proof}
The proof follows from Corollary 1 \citep{tian2002studies}, which states that a node is independent of its ancestors excluding the parents of its $c$-component given the parents of its $c$-component.
\end{proof} 

\textbf{Note.} In a Markovian model there are no bi-directed paths, Therefore, the elementary partition of $\mathcal{A}(Y)$ is the $c$-component of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Therefore, $C_Y = \{Y\}$, and $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}) \backslash\{X\} = \mathcal{P}(Y) \backslash\{X\}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. This matches with our insight in Example 1, where we saw that $Y \perp (\mathcal{A}(Y)\backslash\{X,Y\})\backslash(\mathcal{P}(Y)\backslash\{X\})|(\mathcal{P}(Y)\backslash\{X\})$.

\subsection{Stability of the Solution to Problem \ref{problem:optimal_blocking}} \label{sec:stable_blocking}

We next discuss some concerns with using $\mathcal{Z}^*$ (a solution to \cref{problem:optimal_blocking}) as a blocking set. We provide a method to address those concerns. 

\textbf{Example 4.} In \cref{fig:semi_markovian_model_postxa} and \cref{fig:semi_markovian_model_postxb}, there are some covariates which are ancestors of $Y$ and descendants of $X$. Such covariates are called post-treatment ancestors (excluding itself) of the response. Blocks created using these covariates are not well-defined. For instance, we are interested in studying the causal effect of a drug on blood pressure. Suppose anxiety level mediates the effect of drug on blood pressure, i.e., $\text{drug}\rightarrow\text{anxiety}\rightarrow \text{blood pressure}$. If we create blocks using anxiety then the blocks will change (i.e., become unstable) during the experiment because change in the drug level will cause the anxiety level to change. Therefore, it is reasonable not to create blocks using these covariates. With this insight, for \cref{fig:semi_markovian_model_postxa}, $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_4\}$ blocks all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$. 

However, we cannot simply delete the post-treatment ancestors (excluding itself) of the response from the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ of interest. This is because the presence of latent structures between pre- and post-treatment ancestors of the response affects blocking set of interest. For instance, in \cref{fig:semi_markovian_model_postxb}, $V_1$ is a collider on the path $V_3\rightarrow V_1\leftarrow V_6$. Hence, keeping $V_1$ in the blocking set will open this path for $V_3$ to cause variability in $Y$. Therefore, for  \cref{fig:semi_markovian_model_postxb}, we need $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_3,V_4\}$ to block all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$.

\begin{figure}[t]
\centering
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxa}
\end{minipage}
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [below of=Y] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend right] (Z1) to node {} (Z6);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxb}
\end{minipage}
\caption{Example semi-Markovian models with post-treatment ancestors of $Y$.}\label{fig:semi_markovian_model_postx}
\end{figure}

% To formalize the insight from Example 4, we refer to the following definition.
% \begin{definition} \cite{shpitser2012validity} A causal path from a variable $X \in \mathcal{X}$ to $Y \in \mathcal{Y}$ is called \textit{proper} if it doesn't intersect $\mathcal{X}$ except the endpoints. When $\mathcal{X}$ is a single variable then all causal paths are proper.
% \end{definition}

Denote the post-treatment ancestors (excluding itself) of the response while studying the causal effect $Y|do(X)$ as $\mathcal{M}(Y|do(x))$.
\begin{definition}
For studying the causal effect of $X$ on $Y$, a blocking set $\mathcal{Z}$, is said to be stable if $\mathcal{Z} \cap \mathcal{M}(Y|do(x)) = \phi$.
\end{definition}

Denote the set of descendants (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ as $\mathcal{D}(\cdot)$. %Denote the set of ancestors of $W$ in the subgraph of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ where all edges leaving $X$ as $\mathcal{A}$.
\begin{lemma} \label{lemma:M}
$\mathcal{M}(Y|do(x)) = (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
\end{lemma}
\begin{proof}
The proof follows from the definition of post-treatment ancestors (excluding itself) of $Y$.
\end{proof}

\begin{theorem}\label{theorem:stable_blocking}
A stable solution to \cref{problem:optimal_blocking} is $\mathcal{Z}^* = (\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}} \backslash\{X\}) \backslash \mathcal{M}(Y|do(x))$.
\end{theorem}
\begin{proof}
The proof follows from \cref{lemma:M}.
\end{proof}

%Therefore, we ignore all the variables falling on a proper causal path from $X$ to $Y$. Following \cite{van2014constructing}, the set of all such variables is $Dpcp(X,Y) = De((De_{\widetilde{X}}(X) \backslash X) \cap An_{\tilde{\tilde{X}}(Y))$ where $De(.)$ represents the set of descendants excluding the variable itself and $An_{\tilde{\tilde{X}}(Y)}$ is the ancestral graph of $Y$ where all edges leaving $X$ are removed.

%Note that by definition $Dpcp(X,Y)$ may include non-descendants of $Y$ which we have already argued to not take into consideration in Observation 2. Therefore, we can say that specifically we should not block using  $Dpcp(X,Y)$ in the graph $G_{An_{\widetilde{X}}(Y)}$ denoted as $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}}$. Note that $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}} = Dpcp(X,Y) \cap An_{\widetilde{X}}(Y)$.

\subsection{Final Algorithm}

We next provide steps to obtain a stable solution to \cref{problem:optimal_blocking} based on \cref{theorem:sol_to_optimal_blocking,theorem:sol_to_optimal_blocking_construction,theorem:stable_blocking}. First, we reduce $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Next, we obtain the set $\mathcal{Z} = \mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$ which is the smallest set such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Finally, we drop $\mathcal{M}(Y|do(x))$ from $\mathcal{Z}$ to get a stable solution to \cref{problem:optimal_blocking}.

Denote the edge $W_1\rightarrow W_2$ as \textit{directed-edge}$(W_1,W_2)$, a path consisting of directed edges from $W_1$ to $W_2$ as \textit{directed-path}$(W_1,W_2)$, and a path consisting of all bi-directed edges from $W_1$ to $W_2$ as \textit{bi-directed-path}$(W_1,W_2)$. Algorithm \ref{alg:causal-opt-blocking-set} outlines the psuedocode of the proposed algorithm to obtain a stable solution to \cref{problem:optimal_blocking}.

\begin{algorithm} [!htb]
	\caption{Stable-Causal-Blocking ($\mathcal{G}, X, Y$)}\label{alg:causal-opt-blocking-set}
	\begin{algorithmic}[1]
	    %\State \textbf{Input} {($\mathcal{G}, X, Y$)}.
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}$ to $\mathcal{G}_{\widetilde{X}}$} 
            \If{$\exists$ \textit{directed-edge}($V_i,X$)}
                \State delete \textit{directed-edge}($V_i,X$) from $\mathcal{G}$
            \EndIf
        \EndFor 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X}}$} 
            \If{$\nexists$ \textit{directed-path}($V_i,Y$)}
                \State delete $V_i$ from $\mathcal{G}$
            \EndIf
        \EndFor 
        \State $\mathcal{A}'(Y) \leftarrow \phi$
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}'_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$} 
        \If{$\nexists$ path($V_i,Y$)}
            \State delete $V_i$ from $\mathcal{G}; \mathcal{A}'(Y) \leftarrow \mathcal{A}'(Y) \cup \{V_i\}$
        \EndIf
        \EndFor
        \State $\mathcal{A}(Y) = \mathcal{V}\backslash\mathcal{A}'(Y)$
        \State $\mathcal{S}_i = \{V_i\}, i =1,\dots,|\mathcal{V}|$ \Comment{Finding $C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$}
            \For{$j$ in $1,\dots,i$}
            \If{$\exists$ \textit{bi-directed-path}($V_i$,$V_j$)}
                \State $\mathcal{S}_i \leftarrow \mathcal{S}_i \cup \mathcal{S}_j; \mathcal{S}_j \leftarrow \phi$
            \EndIf
            \EndFor
        \EndFor
        \State $i\leftarrow 1; \mathcal{S} \leftarrow \mathcal{S}_1$
        \While{$Y \notin \mathcal{S}$} 
            \State $i \leftarrow i+1; \mathcal{S} \leftarrow \mathcal{S}_i$
        \EndWhile
        \State $\mathcal{P}(\mathcal{S})=\phi$ \Comment{Finding $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
            \For{$W$ in $\mathcal{S}$}
                \If{$\exists$ \textit{directed-edge}($V_i,W$)}
                    \State $\mathcal{P}(\mathcal{S}) \leftarrow \mathcal{P}(\mathcal{S}) \cup \{V_i\}$
                \EndIf
            \EndFor
        \EndFor 
    	\State $\mathcal{D}(X) \leftarrow \phi$ \Comment{Finding $\mathcal{D}(X)$} 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
        \If{$\nexists$ \textit{directed-path}($X,V_i$)}
            \State $\mathcal{D}(X) \leftarrow \mathcal{D}(X) \cup \{V_i\}$
        \EndIf
        \EndFor    	
    	\State $\mathcal{Z} \leftarrow (\mathcal{P}(\mathcal{S})\backslash\{X\}) \backslash (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
    	\State \textbf{return} $\mathcal{Z}$
	\end{algorithmic}
\end{algorithm}

\subsection{Time Complexity of Algorithm \ref{alg:causal-opt-blocking-set}}
We next show that \cref{alg:causal-opt-blocking-set} is an efficient polynomial-time algorithm. Finding if there exists a path between any two nodes in a directed graph can be done using breath-first-search which has the worst-case time complexity of $O(|\mathcal{V}|^2)$. \cref{alg:causal-opt-blocking-set} first reduces $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ which involves
\begin{enumerate}
    \item finding variables with edges going into $X$: $O(|\mathcal{V}|)$, 
    \item finding variables with no path into $Y$: $O(|\mathcal{V}|^3)$, and 
    \item finding all ancestors of $Y$: $O(|\mathcal{V}|^3)$.
\end{enumerate}
 
\cref{alg:causal-opt-blocking-set} next finds the $c$-component of $Y$ involves traversing all pairs of variables: $O(|\mathcal{V}|^2)$, and finding if there exists a bi-directed path between any pair of variables: $O(|\mathcal{V}|^2)$. Therefore, the total time at this step is $O(|\mathcal{V}|^4)$. Finally \cref{alg:causal-opt-blocking-set} finds $\mathcal{M}(Y|do(x))$ which involves
\begin{enumerate}
    \item finding descendants of $X$: $O(|\mathcal{V}|^3)$, and
    \item finding ancestors of $Y$: $O(|\mathcal{V}|^3)$.
\end{enumerate}

Therefore, the time complexity of \cref{alg:causal-opt-blocking-set} is $O(|\mathcal{V}|^4)$.

\subsection{Implementing Algorithm \ref{alg:causal-opt-blocking-set}}
We demonstrate the implementation of \cref{alg:causal-opt-blocking-set} to obtain a stable solution to \cref{problem:optimal_blocking} for a general semi-Markovian causal graph, $\mathcal{G}$ given in \cref{fig:final_implementation1G}.
\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Z7) [below of=Y] {\scriptsize $V_7$};
  \node[main node] (Z8) [below right of=Z2] {\scriptsize $V_8$};
  \node[main node] (Z9) [above left of=X] {\scriptsize $V_9$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Y) to node {} (Z7);
  \draw[->] (Z1) to node {} (Y);
  \draw[->, bend right] (Z1) to node {} (X);
  \draw[->, bend right] (Z3) to node {} (X);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->, bend left] (Z8) to node {} (Z7);
  \draw[->] (Z9) to node {} (X);
  \draw[->] (Z6) to node {} (Y);
  \draw[->, bend left] (Z2) to node {} (Z7);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Original Graph $\mathcal{G}$.} \label{fig:final_implementation1G}
\end{figure}

\begin{figure}[h!]
\centering
\begin{minipage}{0.42\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Z7) [below of=Y] {\scriptsize $V_7$};
  \node[main node] (Z8) [below right of=Z2] {\scriptsize $V_8$};
  \node[main node] (Z9) [above left of=X] {\scriptsize $V_9$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Y) to node {} (Z7);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z6) to node {} (Y);
  \draw[->, bend left] (Z8) to node {} (Z7);
  \draw[->, bend left] (Z2) to node {} (Z7);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Graph $\mathcal{G}_{\widetilde{X}}$.} \label{fig:figure8}
\end{minipage}
\begin{minipage}{0.42\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize $X$};
  \node[main node] (Z5) [right of=X] {\scriptsize $V_5$};
  \node[main node] (Z6) [below of=Z5] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z5] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Z6) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend right] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Graph $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$.}\label{fig:final_implementation1Gnew}
\end{minipage}
\end{figure}

We first obtain the graph $G_{An_{\widetilde{X}}(Y)}$ as displayed in \cref{fig:final_implementation1Gnew}. We next obtain the $c$-components (following \cref{def:c_component}) of $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$ are $\{X\}, \{V_1,V_5,Y,V_2\}, \{V_3\},\{V_4\}$, and the $c$-component of $Y$ is $\{V_1,V_5,Y,V_2\}$. We next obtain the set of parents of the $c$-component of $Y$ as %$\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\} =
$\{X,V_1,V_2,V_3,V_4,V_5\}$. The set $\mathcal{D}(X) \cap \mathcal{A}(Y)$ is $\{X,Y,V_5,V_6\}$. Finally, we obtain the final set as  $(\{X,V_1,V_2,V_3,V_4,V_5\}\backslash\{X\})\backslash(\{X,Y,V_5,V_6\}\backslash\{X,Y\}) = \{V_1,V_2,V_3,V_4\}$.

==> stable-causal-blocking-arxiv/sections-clear/methodology_v0.02.tex <==
\section{Methodology} \label{sec:methodology}
In this section, we develop a methodology to find a solution to \cref{problem:optimal_blocking}. We first examine $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$ to obviate some edges and nodes from the causal graph, $\mathcal{G}$. We next discuss some motivating examples and make key observations that lead to several lemmas for our main result. In the end, we provide our main result and develop an efficient algorithm for solving \cref{problem:optimal_blocking}.

\subsection{Examining $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}$}
In \cref{problem:optimal_blocking}, our interest is to minimize $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ as a function of $\mathcal{Z}\subseteq \mathcal{C}$. $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ through the causal relationships from $\mathcal{Z}$ to $Y$, and from $\mathcal{Z}$ to $X$. Note that, $X$ is the treatment on which we are performing the intervention, i.e.,  we set the levels/values of $X$. This is equivalent to saying that $X$ is no longer affected by the rest of the variables. Therefore, $\mathcal{Z}$ also cannot affect $X$ when an intervention is performed on $X$. %instead its value is decided/set during the experiment. %In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all arrows coming into $X$. 
Therefore, $\mathcal{Z}$ can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from $\mathcal{Z}$ to $Y$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}$ to $Y$ gives a solution to \ref{problem:optimal_blocking}.

Denote the subgraph of $\mathcal{G}$ where all edges coming into $X$ were deleted as $\mathcal{G}_{\widetilde{X}}$.
\begin{lemma} \label{lemma:Gxbar}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}_{\widetilde{X}}$.
\end{lemma}
\begin{proof}
The proof follows from the fact that when an intervention is performed on $X$ then it is no longer affected by the rest of the variables. In terms of the causal graph, $\mathcal{G}$, it is the same as deleting all edges coming into $X$. 
\end{proof}

\begin{definition}
$\mathcal{S},\mathcal{T}\subseteq \mathcal{C}$ are called equivalent sets (denoted as $\mathcal{S} \equiv \mathcal{T}$), if  $\Var(\hat{\P}_\mathcal{S}(Y|do(X))) = \Var(\hat{\P}_\mathcal{T}(Y|do(X)))$.
\end{definition}

\begin{lemma} \label{lemma:D0}
If $\mathcal{F}$ is the set of all covariates that do not have causal paths to $Y$, then $\mathcal{C}$ and $\mathcal{C}\backslash \mathcal{F}$ are equivalent sets.
\end{lemma}
\begin{proof}
The proof follows from the fact that a set of covariates can affect $\Var(\hat{\P}_\mathcal{Z}(Y|do(X)))$ only through the causal relationships from itself to $Y$. 
\end{proof}
Following \cref{lemma:Gxbar}, we restrict ourselves to the subgraph $\mathcal{G}_{\widetilde{X}}$. Following \cref{lemma:D0}, we further delete the covariates that do not have any causal paths to $Y$. Denote this new subgraph as $\mathcal{G}'_{\widetilde{X}}$ and $\mathcal{C}'=\mathcal{C}\backslash\mathcal{F}$. Therefore, a smallest subset of $\mathcal{C}$ that blocks all causal paths from $\mathcal{C}'$ to $Y$ in $\mathcal{G}'_{\widetilde{X}}$ gives a solution to \ref{problem:optimal_blocking}.

%As discussed earlier, we are interested in performing a randomized experiment to study the causal effect of interest $X\rightarrow Y$ where we are randomizing the treatment $(X)$. In terms of the causal graph, randomizing $X$ is the same as making interventions to set levels/values of $X$. This means that $X$ is not affected by any variable in the graph, instead, its value is decided/set during the experiment. Therefore, we can \textit{ignore all the arrows coming into $X$} and work with the subgraph of $G$ where all arrows coming into $X$ are ignored. We denote such subgraph as $G_{\widetilde{X}}$. Therefore, for the examples, we work with causal graphs with no arrows coming to $X$.

\subsection{Motivating Examples and Key Observations}

All causal graphs in \cref{fig:markovian_model,fig:semi_markovian_model_C,fig:semi_markovian_model_Y,fig:semi_markovian_model_des,fig:semi_markovian_model_postx} represent $\mathcal{G}'_{\widetilde{X}}$. Denote the set of parents of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{P}(W)$.

\begin{note}
\textup{In all the graphs provided in this paper, a bi-directed edge between any two observed variables is the same as those two variables having one or more unobserved ancestors. For example $V_3 \dashleftarrow \dashrightarrow V_4$ is the same as $V_3 \dashleftarrow U \dashrightarrow V_4$ for some unobserved variable, $U$.
}
\end{note}

\begin{example} \label{example:1} 
\textup{
For \cref{fig:markovian_model,fig:semi_markovian_model_C}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. Therefore, $\mathcal{Z}^* = \mathcal{P}(Y)\backslash\{X\}$.}
\end{example}

\begin{figure}[th]
\centering
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.7cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  
  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \end{scope}
\end{tikzpicture}
\caption{Example Markovian model (no latent structures).} \label{fig:markovian_model}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.40\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize  $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.7cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed] (Z3) to node {} (Z4);
  \end{scope}
\end{tikzpicture}
\caption{Example semi-Markovian model with latent variables involving only $\mathcal{C}'$.} \label{fig:semi_markovian_model_C}
\end{minipage}
\end{figure}

\begin{example} \label{example:2} 
\textup{
For \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{P}(Y)\backslash\{X\}=\{V_1,V_2\}$ is not sufficient to block all causal paths from $\mathcal{C}'=\{V_1,V_2,V_3,V_4\}$ to $Y$. In \cref{fig:semi_markovian_model_Ya}, the reason is that blocking using $V_2$ opens the path $V_4 \rightarrow V_2 \dashleftarrow \dashrightarrow Y$ for $V_4$ to cause variability in $Y$. In \cref{fig:semi_markovian_model_Yb}, the reason is that the latent structure $Y \dashleftarrow \dashrightarrow V_4$ enables $V_4$ to cause $Y$ even when the path $V_4\rightarrow V_2\rightarrow Y$ is blocked. For both \cref{fig:semi_markovian_model_Ya,fig:semi_markovian_model_Yb}, $\mathcal{Z}^*=(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$.
}
\end{example}

\begin{figure}[thb]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Ya}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[<->, densely dashed] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_Yb}
\end{minipage}\hspace{.5cm}
\caption{Example semi-Markovian model with latent variables involving $\mathcal{C}'$ and $Y$.}\label{fig:semi_markovian_model_Y}
\end{figure}

\begin{definition} \label{def:collider} \citep{pearl2009causality,rohrer2018thinking}
A variable is a collider or an inverted fork when it is causally influenced by two or more variables.
\end{definition}

\begin{note}
\textup{
If we condition/block using a collider (and/or it's descendants) then the common causes of the collider become statistically dependent \citep{berkson1946limitations,cole2010illustrating}. For example, if alcohol and smoking are common causes of high blood pressure then it is not necessary that these common causes are correlated in the population at large. However, if we restrict our attention to (condition on) those with high blood pressure then we introduce a non-causal dependence between alcohol and smoking. \footnote{The reader may refer to the tutorials \href{https://www.col-ex.org/posts/conditioning-causal-graphs/\#d-separation-and-d-connection-along-a-path}{Collectively Exhaustive} and \href{https://donskerclass.github.io/CausalEconometrics/DAGs.html}{Causal Graphs by David Childers} for understanding the basic concepts related to causal graphs.}
}
\end{note} 

\begin{example} \label{example:3} 
\textup{
For \cref{fig:semi_markovian_model_des}, despite $Y$ having descendants, $(\mathcal{P}(Y)\backslash\{X\}) \cup \{V_4\}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. This is because descendants of $Y$ can never be a cause of variability in $Y$. In \cref{fig:semi_markovian_model_desa,fig:semi_markovian_model_desb}, $V_5$ (a descendant of $Y$) cannot cause $Y$ through the edge $Y \rightarrow V_5$. Moreover, $V_4$ (an ancestor of $Y$) cannot cause $Y$ through $V_5$ because $V_5$ is a collider on the path $V_4\rightarrow V_5 \leftarrow Y$.
}
\end{example}

\begin{figure}[th]
\centering
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [right of=Y, node distance=1.1cm] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[->, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desa}
\end{minipage}\hspace{.5cm}
\begin{minipage}{.30\textwidth}
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Y)  [right of=X] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z5) [ right of=Y, node distance=1.1cm] {\scriptsize $V_5$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};

  \begin{scope}
  \draw[->] (X) to node {} (Y);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Y) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_desb}
\end{minipage}
\caption{Example Semi-Markovian Models with latent variables involving $\mathcal{C}'$ and $Y$, and $Y$ having descendants.}\label{fig:semi_markovian_model_des}
\end{figure}

Denote the set of ancestors (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X}}$ as $\mathcal{A}(W)$. Denote the subgraph of $\mathcal{G}'_{\widetilde{X}}$ restricted to $\mathcal{A}(Y)$ as $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Based on the insights from \cref{example:1,example:2,example:3}, we write \cref{lemma:GxbarA}.
\begin{lemma}\label{lemma:GxbarA}
For finding a solution to \cref{problem:optimal_blocking}, it is sufficient to work with the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$.
\end{lemma}

\begin{proof}
The proof follows from the fact the graph under consideration is acyclic. Hence, the descendants of a node can never be its causes even in the presence of latent structures.
\end{proof}

\subsection{Solution to Problem \ref{problem:optimal_blocking}}

We now combine the insights from \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA} to provide a solution to \cref{problem:optimal_blocking}.

\begin{theorem} \label{theorem:sol_to_optimal_blocking}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ is a solution to \cref{problem:optimal_blocking}.
\end{theorem}
\begin{proof}
The proof follows from the fact that $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ blocks all causal paths from $\mathcal{C}'$ to $Y$. %following \cref{lemma:Gxbar,lemma:D0,lemma:GxbarA}.
\end{proof}

\cref{theorem:sol_to_optimal_blocking} provides a sufficient condition for a set $\mathcal{Z}$ to be a solution to \cref{problem:optimal_blocking}. We next provide a method to construct a set $\mathcal{Z}$ that satisfies this sufficient condition.

Let a path composed entirely of bi-directed edges be called a \textit{bi-directed path}.
\begin{definition}\label{def:c_component} \citep{tian2002general}. 
For a graph $\mathcal{G}$, the set of observed variables $\mathcal{V}$, can be \textit{partitioned} into disjoint groups by assigning two variables to the same group if and only if they are connected by a bi-directed path. Assume that $V$ is therefore partitioned into $k$ groups $\mathcal{S}_1, \dots, \mathcal{S}_k$. We will call each $\mathcal{S}_j; j=1, \dots, k,$ a \textit{$c$-component} of $V$ in $\mathcal{G}$ or a $c$-component (abbreviating confounded component) of $\mathcal{G}$. The $\mathcal{S}_j$ such that $W\in S_j$ is called the \textit{$c$-component of $W$} in $\mathcal{G}$ and is denoted as $C_{W,\mathcal{G}}$. As $\{\mathcal{S}_1, \dots, \mathcal{S}_k\}$ is a partition of $\mathcal{V}$, $c$-component of a variable always exists and is unique.
\end{definition}

In \cref{example:2}, we observed that due to the presence of latent structures involving $Y$, $\mathcal{P}(Y)$ was not sufficient to block all causal paths from $\mathcal{C}'$ to $Y$. However the parents of $c$-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ would be sufficient for that purpose. 

\begin{theorem} \label{theorem:sol_to_optimal_blocking_construction}
The smallest $\mathcal{Z}$ such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ is  the set of parents of c-component of $Y$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ excluding $X$ denoted as $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$.
\end{theorem} 
\begin{proof}
The proof follows from Corollary 1 \citep{tian2002studies}, which states that a node is independent of its ancestors excluding the parents of its $c$-component given the parents of its $c$-component.
\end{proof} 

\begin{note} 
\textup{
In a Markovian model there are no bi-directed paths, Therefore, the elementary partition of $\mathcal{A}(Y)$ is the $c$-component of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Therefore, $C_Y = \{Y\}$, and $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}) \backslash\{X\} = \mathcal{P}(Y) \backslash\{X\}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. This matches with our insight in \cref{example:1}, where we observed that $Y \perp (\mathcal{A}(Y)\backslash\{X,Y\})\backslash(\mathcal{P}(Y)\backslash\{X\})|(\mathcal{P}(Y)\backslash\{X\})$.
}
\end{note}

\subsection{Stability of the Solution to Problem \ref{problem:optimal_blocking}} \label{sec:stable_blocking}

We next discuss some concerns with using $\mathcal{Z}^*$ (a solution to \cref{problem:optimal_blocking}) as a blocking set. We provide a method to address those concerns. 
\begin{definition} \label{def:ptay}
Post-treatment ancestors of  (excluding $X$) of the response are those ancestors of  (excluding $X$) of the response who are also the descendants of the treatment.
\end{definition}

Denote the post-treatment ancestors of the response while studying the causal effect $Y|do(X)$ as $\mathcal{M}(Y|do(X))$, and the set of descendants (including itself) of $W$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ as $\mathcal{D}(W)$.

%Post-treatment ancestors (excluding itself) of the response are those ancestors (excluding itself) of the response who are also the descendants of the treatment. 
%Denote the set of ancestors of $W$ in the subgraph of $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ where all edges leaving $X$ as $\mathcal{A}$.
\begin{lemma} \label{lemma:M}
$\mathcal{M}(Y|do(X)) = (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
\end{lemma}
\begin{proof}
The proof follows directly from \cref{def:ptay}. %i.e. post-treatment ancestors (excluding itself) of $Y$.
\end{proof}


\begin{example} \label{example:4} 
\textup{In \cref{fig:semi_markovian_model_postxa,fig:semi_markovian_model_postxb}, there exist post-treatment ancestors (excluding itself) of the response. Blocks created using these covariates are not well-defined. For instance, we are interested in studying the causal effect of a drug on blood pressure. Suppose anxiety level mediates the effect of drug on blood pressure, i.e., $\text{drug}\rightarrow\text{anxiety}\rightarrow \text{blood pressure}$. If we create blocks using anxiety then the blocks will change (i.e., become unstable) during the experiment because change in the drug level will cause the anxiety level to change. Therefore, it is reasonable not to create blocks using these covariates. With this insight, for \cref{fig:semi_markovian_model_postxa}, $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_4\}$ blocks all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$.  However, we cannot simply delete the post-treatment ancestors (excluding itself) of the response from the subgraph $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ of interest. This is because the presence of latent structures between pre- and post-treatment ancestors of the response affects blocking set of interest. For instance, in \cref{fig:semi_markovian_model_postxb}, $V_1$ is a collider on the path $V_3\rightarrow V_1\leftarrow V_6$. Hence, keeping $V_1$ in the blocking set will open this path for $V_3$ to cause variability in $Y$. Therefore, for \cref{fig:semi_markovian_model_postxb}, we need $(\mathcal{P}(Y)\backslash\{X\})\cup\{V_3,V_4\}$ to block all (pre-treatment) causal paths from $\mathcal{C}'$ to $Y$.
}
\end{example}

\begin{figure}[t]
\centering
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [right of=Y, node distance=1.1cm] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxa}
\end{minipage}
\begin{minipage}{.30\textwidth}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X)  [] {\scriptsize $X$};
  \node[main node] (Z6) [right of=X] {\scriptsize $V_6$};
  \node[main node] (Y)  [right of=Z6] {\scriptsize $Y$};
  \node[main node] (Z1) [above of=Y] {\scriptsize $V_1$};
  \node[main node] (Z2) [right of=Z1, node distance=.6cm] {\scriptsize $V_2$};
  \node[main node] (Z3) [above left of=Z1] {\scriptsize $V_3$};
  \node[main node] (Z4) [above right of=Z2] {\scriptsize $V_4$};
  \node[main node] (Z5) [right of=Y, node distance=1.1cm] {\scriptsize $V_5$};
  \node[main node] (Z7) [below of=Z6] {\scriptsize $V_7$};

  \begin{scope}
  \draw[->] (X) to node {} (Z6);
  \draw[->] (Y) to node {} (Z5);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->] (Z3) to node {} (Z1);
  \draw[->] (Z6) to node {} (Z7);
  \draw[->] (Z6) to node {} (Y);  
  \draw[->] (Z4) to node {} (Z2); 
  \draw[->] (Z7) to node {} (Y); 
  \draw[<->, densely dashed, bend right] (Z1) to node {} (Z6);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Z5);
  \draw[<->, densely dashed, bend left] (Z3) to node {} (Z4);
  \draw[<->, densely dashed, bend left] (Z4) to node {} (Y);
  \end{scope}
\end{tikzpicture}
\subcaption{}\label{fig:semi_markovian_model_postxb}
\end{minipage}
\caption{Example semi-Markovian models with post-treatment ancestors of $Y$.}\label{fig:semi_markovian_model_postx}
\end{figure}

% To formalize the insight from Example 4, we refer to the following definition.
% \begin{definition} \cite{shpitser2012validity} A causal path from a variable $X \in \mathcal{X}$ to $Y \in \mathcal{Y}$ is called \textit{proper} if it doesn't intersect $\mathcal{X}$ except the endpoints. When $\mathcal{X}$ is a single variable then all causal paths are proper.
% \end{definition}


\begin{definition}
For studying the causal effect of $X$ on $Y$, a blocking set $\mathcal{Z}$, is said to be stable if $\mathcal{Z} \cap \mathcal{M}(Y|do(X)) = \phi$.
\end{definition}

\begin{theorem}\label{theorem:stable_blocking}
A stable solution to \cref{problem:optimal_blocking} is $\mathcal{Z}^* = (\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}} \backslash\{X\}) \backslash \mathcal{M}(Y|do(X))$.
\end{theorem}
\begin{proof}
The proof follows from \cref{lemma:M}.
\end{proof}

%Therefore, we ignore all the variables falling on a proper causal path from $X$ to $Y$. Following \cite{van2014constructing}, the set of all such variables is $Dpcp(X,Y) = De((De_{\widetilde{X}}(X) \backslash X) \cap An_{\tilde{\tilde{X}}(Y))$ where $De(.)$ represents the set of descendants excluding the variable itself and $An_{\tilde{\tilde{X}}(Y)}$ is the ancestral graph of $Y$ where all edges leaving $X$ are removed.

%Note that by definition $Dpcp(X,Y)$ may include non-descendants of $Y$ which we have already argued to not take into consideration in Observation 2. Therefore, we can say that specifically we should not block using  $Dpcp(X,Y)$ in the graph $G_{An_{\widetilde{X}}(Y)}$ denoted as $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}}$. Note that $Dpcp(X,Y)_{G_{An_{\widetilde{X}}(Y)}} = Dpcp(X,Y) \cap An_{\widetilde{X}}(Y)$.

\subsection{Final Algorithm}

We next provide steps to obtain a stable solution to \cref{problem:optimal_blocking} based on \cref{theorem:sol_to_optimal_blocking,theorem:sol_to_optimal_blocking_construction,theorem:stable_blocking}. First, we reduce $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Next, we obtain the set $\mathcal{Z} = \mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\}$ which is the smallest set such that $Y \perp (\mathcal{A}(Y)\backslash \{X,Y\})\backslash\mathcal{Z}|\mathcal{Z}$ in $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$. Finally, we drop $\mathcal{M}(Y|do(X))$ from $\mathcal{Z}$ to get a stable solution to \cref{problem:optimal_blocking}.

Denote the edge $W_1\rightarrow W_2$ as \textit{directed-edge}$(W_1,W_2)$, a path consisting of directed edges from $W_1$ to $W_2$ as \textit{directed-path}$(W_1,W_2)$, and a path consisting of all bi-directed edges from $W_1$ to $W_2$ as \textit{bi-directed-path}$(W_1,W_2)$. Algorithm \ref{alg:causal-opt-blocking-set} outlines the psuedocode of the proposed algorithm to obtain a stable solution to \cref{problem:optimal_blocking}.

% \if 0
\begin{algorithm} [!htb]
	\caption{Stable-Causal-Blocking ($\mathcal{G}, X, Y$)}\label{alg:causal-opt-blocking-set}
	\begin{algorithmic}[1]
	    %\State \textbf{Input} {($\mathcal{G}, X, Y$)}.
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}$ to $\mathcal{G}_{\widetilde{X}}$} 
            \If{$\exists$ \textit{directed-edge}($V_i,X$)}
                \State delete \textit{directed-edge}($V_i,X$) from $\mathcal{G}$
            \EndIf
        \EndFor 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X}}$} 
            \If{$\nexists$ \textit{directed-path}($V_i,Y$)}
                \State delete $V_i$ from $\mathcal{G}$
            \EndIf
        \EndFor 
        \State $\mathcal{A}(Y) \leftarrow \{Y\}$
        \For{$i$ in $1,\dots,|\mathcal{V}|$} \Comment{Reducing $\mathcal{G}'_{\widetilde{X}}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$} 
        \If{$\exists$ path($V_i,Y$)}
            \State $\mathcal{A}(Y) \leftarrow \mathcal{A}(Y) \cup \{V_i\}$
        \EndIf
        \EndFor
        %\State $\mathcal{A}(Y) = \mathcal{V}\backslash\mathcal{A}'(Y)$
        \State $\mathcal{S}_i = \{V_i\}, i =1,\dots,|\mathcal{V}|$ \Comment{Finding $C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}}$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$}
            \For{$j$ in $1,\dots,i$}
            \If{$\exists$ \textit{bi-directed-path}($V_i$,$V_j$)}
                \State $\mathcal{S}_i \leftarrow \mathcal{S}_i \cup \mathcal{S}_j; \mathcal{S}_j \leftarrow \phi$
            \EndIf
            \EndFor
        \EndFor
        \State $i\leftarrow 1; \mathcal{S} \leftarrow \mathcal{S}_1$
        \While{$Y \notin \mathcal{S}$} 
            \State $i \leftarrow i+1; \mathcal{S} \leftarrow \mathcal{S}_i$
        \EndWhile
        \State $\mathcal{P}(\mathcal{S})=\phi$ \Comment{Finding $\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})$}
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
            \For{$W$ in $\mathcal{S}$}
                \If{$\exists$ \textit{directed-edge}($V_i,W$)}
                    \State $\mathcal{P}(\mathcal{S}) \leftarrow \mathcal{P}(\mathcal{S}) \cup \{V_i\}$
                \EndIf
            \EndFor
        \EndFor 
    	\State $\mathcal{D}(X) \leftarrow \{X\}$ \Comment{Finding $\mathcal{D}(X)$} 
        \For{$i$ in $1,\dots,|\mathcal{V}|$} 
        \If{$\exists$ \textit{directed-path}($X,V_i$)}
            \State $\mathcal{D}(X) \leftarrow \mathcal{D}(X) \cup \{V_i\}$
        \EndIf
        \EndFor  
        %\State $\mathcal{D}(X) = \mathcal{V}\backslash\mathcal{D}'(X)$
    	\State $\mathcal{Z} \leftarrow (\mathcal{P}(\mathcal{S})\backslash\{X\}) \backslash (\mathcal{D}(X) \cap \mathcal{A}(Y))\backslash \{X,Y\}$.
    	\State \textbf{return} $\mathcal{Z}$
	\end{algorithmic}
\end{algorithm}
% \fi

\subsection{Time Complexity of Algorithm \ref{alg:causal-opt-blocking-set}}
We next show that \cref{alg:causal-opt-blocking-set} is an efficient polynomial-time algorithm. Finding if there exists a path between any two nodes in a directed graph can be done using breath-first-search which has the worst-case time complexity of $O(|\mathcal{V}|^2)$. \cref{alg:causal-opt-blocking-set} first reduces $\mathcal{G}$ to $\mathcal{G}'_{\widetilde{X},\mathcal{A}(Y)}$ which involves finding variables with edges going into $X$ taking $O(|\mathcal{V}|)$ steps, finding variables with no path into $Y$ taking $O(|\mathcal{V}|^3)$ steps, and finding all ancestors of $Y$ taking $O(|\mathcal{V}|^3)$ steps. \cref{alg:causal-opt-blocking-set} next finds the $c$-component of $Y$ involves traversing all pairs of variables: $O(|\mathcal{V}|^2)$, and finding if there exists a bi-directed path between any pair of variables: $O(|\mathcal{V}|^2)$. Therefore, the total time at this step is $O(|\mathcal{V}|^4)$. Finally \cref{alg:causal-opt-blocking-set} finds $\mathcal{M}(Y|do(X))$ which involves finding descendants of $X$ taking $O(|\mathcal{V}|^3)$ steps, and finding ancestors of $Y$ taking $O(|\mathcal{V}|^3)$ steps. Therefore, the time complexity of \cref{alg:causal-opt-blocking-set} is $O(|\mathcal{V}|^4)$.

% \begin{enumerate}
%     \item finding variables with edges going into $X$: $O(|\mathcal{V}|)$, 
%     \item finding variables with no path into $Y$: $O(|\mathcal{V}|^3)$, and 
%     \item finding all ancestors of $Y$: $O(|\mathcal{V}|^3)$.
% \end{enumerate}
 

% \begin{enumerate}
%     \item finding descendants of $X$: $O(|\mathcal{V}|^3)$, and
%     \item finding ancestors of $Y$: $O(|\mathcal{V}|^3)$.
% \end{enumerate}



\subsection{Implementing Algorithm \ref{alg:causal-opt-blocking-set}} \label{sec:implementingthealgo}
We demonstrate the implementation of \cref{alg:causal-opt-blocking-set} to obtain a stable solution to \cref{problem:optimal_blocking} for a general semi-Markovian causal graph, $\mathcal{G}$ given in \cref{fig:final_implementation1G}.

\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize Drug ($X$)};
  \node[main node] (Z5) [right of=X, node distance = 2cm] {\scriptsize Anxiety};
  \node[main node] (Y)  [right of=Z5, node distance = 3cm] {\scriptsize Blood Pressure ($Y$)};
  \node[main node] (Z1) [above of=Y] {\scriptsize Alcohol};
  \node[main node] (Z2) [right of=Z1, node distance = 3cm] {\scriptsize Cholesterol};
  \node[main node] (Z3) [above of=X] {\scriptsize Food-Habits};
  \node[main node] (Z4) [right of=Z2, node distance = 2cm] {\scriptsize Age};
  \node[main node] (Z6) [below of=Z5] {\scriptsize Sleep-Quality};
  \node[main node] (Z7) [below of=Y] {\scriptsize Palpitations};
  \node[main node] (Z8) [right of=Z7, node distance = 3cm] {\scriptsize Strenuous-Activity};
  \node[main node] (Z9) [left of=X, node distance = 2.5cm] {\scriptsize Blood-Sugar};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Y) to node {} (Z7);
  \draw[->] (Z1) to node {} (Y);
  \draw[->, bend right] (Z1) to node {} (X);
  \draw[->] (Z3) to node {} (X);
  \draw[->] (Z2) to node {} (Y);
  \draw[->, bend left] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z8) to node {} (Z7);
  \draw[->] (Z9) to node {} (X);
  \draw[->] (Z6) to node {} (Y);
  \draw[->, bend left] (Z2) to node {} (Z7);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Original Graph $\mathcal{G}$.} \label{fig:final_implementation1G}
\end{figure}

\if 0
\begin{figure}[h!]
\centering
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1cm,thin,main node/.style={font=\sffamily\small\bfseries}]
  \title{Figure 1}
  \node[main node] (X) {\scriptsize Drug ($X$)};
  \node[main node] (Z5) [right of=X, node distance = 2cm] {\scriptsize Anxiety};
  \node[main node] (Y)  [right of=Z5, , node distance = 3cm] {\scriptsize Blood Pressure ($Y$)};
  \node[main node] (Z1) [above of=Y] {\scriptsize Alcohol};
  \node[main node] (Z2) [right of=Z1, node distance = 3cm] {\scriptsize Cholesterol};
  \node[main node] (Z3) [left of=Z1, node distance = 4cm] {\scriptsize Food-Habits};
  \node[main node] (Z4) [right of=Z2, node distance = 2cm] {\scriptsize Age};
  \node[main node] (Z6) [below of=Z5] {\scriptsize Sleep-Quality};
  
  \begin{scope}
  \draw[->] (X) to node {} (Z5);
  \draw[->] (Z5) to node {} (Y);
  \draw[->] (Z5) to node {} (Z6);
  \draw[->] (Z1) to node {} (Y);
  \draw[->] (Z2) to node {} (Y);
  \draw[->, bend left] (Z3) to node {} (Z1);
  \draw[->] (Z4) to node {} (Z2);
  \draw[->] (Z6) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z2) to node {} (Y);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Z1);
  \draw[<->, densely dashed, bend left] (Z5) to node {} (Y);
  \end{scope}  
\end{tikzpicture}
\caption{The Graph $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$.}\label{fig:final_implementation1Gnew}
\end{figure}
\fi

We first obtain the graph $G_{An_{\widetilde{X}}(Y)}$. %as displayed in \cref{fig:final_implementation1Gnew}. 
We next obtain the $c$-components (following \cref{def:c_component}) of $\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}$ are $\{X\}, \{\text{Alcohol}, \text{Anxiety}, Y, \text{Cholesterol}\}, \{\text{Food-Habits}\}, \{\text{Age}\}$, and the $c$-component of $Y$ is $\{\text{Alcohol},\text{Anxiety},Y,\text{Cholesterol}\}$. We next obtain the set of parents of the $c$-component of $Y$ as %$\mathcal{P}(C_{Y,\mathcal{G}_{\widetilde{X},\mathcal{A}(Y)}})\backslash\{X\} =
$\{X, \text{Alcohol}, \text{Cholesterol}, \text{Food-Habits}, \text{Age}, \text{Anxiety}\}$. The set $\mathcal{D}(X) \cap \mathcal{A}(Y)$ is $\{X,Y,\text{Anxiety},\text{Sleep-Quality}\}$. Finally, we obtain the final set as:
$$(\{X, \text{Alcohol}, \text{Cholesterol}, \text{Food-Habits}, \text{Age}, \text{Anxiety}\}\backslash\{X\})\backslash(\{X,Y,\text{Anxiety},\text{Sleep-Quality}\}\backslash\{X,Y\})$$ 
$$= \{\text{Alcohol}, \text{Cholesterol}, \text{Food-Habits}, \text{Age}\}.$$

==> stable-causal-blocking-arxiv/sections-clear/problem_formulation.tex <==
\section{Background and Problem Formulation} \label{sec:prob_formulation}

%Consider a \textit{structural causal model} \citetp{pearl2009causality} $M=\{U,V,F\}$, where $U$ is the set of exogenous variables, $V$ is the set of endogenous variables and $F$ is the set of functions controlling the causal structure. 

In this section, we provide some background and formulate the problem of interest in this paper.

Let $\mathcal{V}$ be the set of observed random variables and $\mathcal{U}$ be the set of unobserved random variables. Let $\mathcal{G}$ be a directed acyclic graph that depicts the causal relationships among the random variables in $\mathcal{U}$ and $\mathcal{V}$. Formally, we are assuming that the probability distribution of the random variables in $\mathcal{U}$ and $\mathcal{V}$ factorizes according to $\mathcal{G}$ (the causal Markov condition \citep{geiger1990logic}). Furthermore, we assume that no variables other than the ones that are $d$-separated \citep{pearl2009causality} in $\mathcal{G}$ are independent, i.e. independence in the joint probability distribution of the random variables in $\mathcal{U}$ and $\mathcal{V}$ is encoded by the causal graph (the causal faithfulness condition \citep{meek1995strong}).

We are interested in studying the causal effect of $X\in\mathcal{V}$ (treatment) on $Y\in\mathcal{V}$ (response). Studying the causal effect of $X$ on $Y$ means learning the (interventional) probability distribution, $\mathbb{P}(Y|do(X))$ \citep{pearl2009causality}.

\subsection{Gain in Precision due to Blocking} \label{sec:gain_in_precision}
Consider a simple setting where $X$ is an indicator random variable defined as
\begin{equation}
X = 
\begin{cases} 
    1, & \text{if the treatment is applied}, \\
    0, & \text{otherwise,}
\end{cases}
\end{equation}
and $Y$ is a real-valued random variable.

Let there be $n$ experimental units available to study the causal effect of $X$ on $Y$ by performing a randomized experiment. Let $\mathcal{Z}$ denote the set of covariates that vary across the experimental units. 

We want to demonstrate the gain in precision due to blocking. Thus, we first ignore these covariates and perform a CRD as follows. We randomize $X$ over the available experimental units, i.e., randomly assign a unit to either have the treatment ($X=1$) or not ($X=0$) and then observe the response. Let $(X_i,Y_i)$ denote the treatment and response pair for the $i$th experimental unit. %As different units are identical and we have randomized the treatment, $X_i$ and $Y_i$ are nothing but i.i.d. copies of $X$ and $Y$, respectively. In other words, $\{(X_i,Y_i): i=1,\dots,n\}$ is a random sample from ($X,Y$). 
Define $I_x:=\{i:X_i=x\}$ and $n_x:=|I_x|$. 

%denote the set of indices of units where the value of treatment, and $I_1:=\{i:X_i=0\}$ denote the set of indices of units where the treatment is not applied. Further, define $n_1:=|I_1|$ and $n_0:=|I_0|$.

%For demonstrating 
To demonstrate the gain in precision due to blocking, we focus on estimating $\mathbb{E}(Y|do(X))$. For simplicity, define $Y(x) := Y|do(X=x)$. For our simple setting, we have only two possibilities of that conditional expectation, viz. $\mathbb{E}(Y(1))$ and $\mathbb{E}(Y(0))$.  Similar to \citet{heckman1992randomization}, \citet{clements1994making}, and \citet{heckman1995assessing}, we define the \textit{effect of treatment} (ET) or \textit{average treatment effect} (ATE) in the population as
\begin{align}
\beta := \E(Y(1)) - \E(Y(0)). \label{eq:beta}
\end{align}

A natural non-parametric estimator of $\E(Y(x))$ is the corresponding sample average, given as
\begin{align}
\bar{Y}(x) &:= \frac{1}{n_x}\sum_{i\in I_x}Y_{i}.
\end{align}
Therefore, we can estimate $\beta$ as
\begin{align}
\hat{\beta} &= \bar{Y}(1) - \bar{Y}(0)
\end{align}

It can be shown that $\mathbb{E}(\hat{\beta}) = \beta$, i.e., $\hat{\beta}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{n_{1,z}} + \frac{\Var(Y(0)|\mathcal{Z})}{n_{0,z}} \right) + \mathbb{E}_\mathcal{Z}(\beta(\mathcal{Z})-\beta)^2, \label{eq:var_under_no_blocking}
\end{align}
where $\beta(\mathcal{Z}):= \E(Y(1)|\mathcal{Z}) - \E(Y(0)|\mathcal{Z})$ is called the \textit{$\mathcal{Z}$-specific causal effect} or \textit{conditional average treatment effect} (CATE). For proofs of unbiasedness and variance of $\hat{\beta}$, refer to \cref{app:proofs_hat_beta}.

We now perform an RBD as follows. We first stratify the experimental units such that units within each stratum (known as a block) are identical, i.e., the covariates in $\mathcal{Z}$ remain the same with a block. We next randomize $X$ over the experimental units within each block and then observe the response. Let $(X_i,Y_i,\mathcal{Z}_i)$ denote the treatment, response, and covariates triplet for the $i$th experimental unit. Define $I_{x,z}:=\{i:X_i=x,\mathcal{Z}_i = z\}$ and $n_{x,z}:=|I_{x,z}|$. 

Following \citep{petersen2006estimation}, ET defined in \eqref{eq:beta} can be re-written as 
\begin{align}
    \beta &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}\right) - \E_\mathcal{Z}\left(\E(Y(0) | \mathcal{Z}\right),\\
    &= \E_\mathcal{Z}\left(\E(Y(1) | \mathcal{Z}) - \E(Y(0) | \mathcal{Z})\right), \\
    &= \sum_{\mathcal{Z}} \left(\E(Y(1) | \mathcal{Z}) - \E(Y(0) | \mathcal{Z}) \right) \P(\mathcal{Z}) \label{eq:beta_z}
\end{align}
A natural non-parametric estimator of $\E(Y(x)|\mathcal{Z})$ is the corresponding sample average, given as
\begin{align}
    \bar{Y}(x)|\mathcal{Z} &:= \frac{1}{n_{x,z}}\sum_{i\in I_{x,z}} Y_i
\end{align}
Define $n_z:=n_{1,z} + n_{0,z}$. $\P(\mathcal{Z})$ can be estimated as
\begin{align}
    \hat{\P}(\mathcal{Z}) &:= \frac{n_z}{n} 
\end{align}
Therefore, we can estimate $\beta$ as
\begin{align}
\hat{\beta}_\mathcal{Z} &= \frac{1}{n}\sum_{\mathcal{Z}} n_{z} \left(\bar{Y}(1) | \mathcal{Z} - \bar{Y}(0) | \mathcal{Z} \right) \label{eq:hat_beta_z}
\end{align}
It can be shown that $\mathbb{E}(\hat{\beta}_\mathcal{Z}) = \beta$, i.e., $\hat{\beta}_\mathcal{Z}$ is \textit{unbiased} for $\beta$. The variance of $\hat{\beta}_\mathcal{Z}$ is given as follows.
\begin{align}
    \Var(\hat{\beta}_\mathcal{Z}) = 
      \mathbb{E}_\mathcal{Z}\left(\frac{\Var(Y(1)|\mathcal{Z})}{n_{1,z}} + \frac{\Var(Y(0)|\mathcal{Z})}{n_{0,z}} \right) + \mathbb{E}_\mathcal{Z}\left(\sum_{\mathcal{Z}}\beta(\mathcal{Z})\hat{\P}(\mathcal{Z}) - \beta \right)^2, \label{eq:var_under_blocking}
\end{align}
For proofs of unbiasedness and variance of $\hat{\beta}_\mathcal{Z}$, refer to \cref{app:proofs_hat_betaz}.

As $\hat{\mathbb{P}}(\mathcal{Z})$ is as an unbiased estimate of $\mathbb{P}(\mathcal{Z})$, $\sum_{\mathcal{Z}}\beta(\mathcal{Z})\hat{\P}(\mathcal{Z}) = \mathbb{E}_\mathcal{Z}(\beta(\mathcal{Z})) = \beta$. Hence, the second term on the right in \eqref{eq:var_under_blocking} is zero. By comparing \eqref{eq:var_under_no_blocking} and \eqref{eq:var_under_blocking}, we observe that $\Var(\hat{\beta}_\mathcal{Z}) \le \Var(\hat{\beta})$, i.e., blocking improves the precision of the estimate of the population average causal effect. %, $\beta$.

\begin{note}
\textup{Blocking is guaranteed to reduce the variance of the estimates of the causal effects under the condition the experimental units are homogeneous within each block and heterogeneous across different blocks. If the blocks are formed using some covariates that do not ensure this then blocking may, in fact, increase the variance. Hence, in practice, blocking involves a trade-off as it partitions the experimental units and thus reduces the sample size for estimating the within-block causal effect which increases the variance but may reduce the inherent variability of the response within each block which can reduce the variance. %Hence, in practice forming blocks using meaningless variables may, in fact, increase the variance.
}
\end{note}

%Another example to demonstrate the gain in precision due to blocking is as follows. Suppose there are $k$ treatments and $b$ blocks, then the response can be defined as a linear equation: $y_{ij} = \mu + \tau_i + b_j + \epsilon_{ij}$, where $\mu$ is the general mean effect, $\tau_i$ is the effect due to the $i$th treatment, $b_j$ is the effect due to the $j$th block, and $\epsilon_{ij}$ is the noise or the experimental error. Clearly, in the absence of $b_j$, the error is higher as compared to the case when $b_j$ is there.

%If the experimental units are identical then $\hat{\beta}_\mathcal{Z} = \hat{\beta}$. 

%\textbf{Remark.} Suppose there are no units in one or more blocks, i.e., $n_{x,z} = 0$ for some $z$, then the overall average treatment effect can be estimated but the $z$-specific causal effect cannot be estimated. Therefore, it is desirable to have units in every block. This also rules out the argument against randomized block experiments that matching of units can be done post a completely randomized experiment based on the covariates, as it is possible that there are no units corresponding to a particular covariate combination.

%\subsection{Gain in Precision under Blocking} We have seen that blocking improves the precision of the estimates. Sometimes, the interest is to study the causal effects from the observational data, a possibility because carrying out a randomized experiment is either economically or ethically infeasible. An approach similar to blocking (in randomized experiments) called \textit{matching} is used to study the causal effects from the observational data, where the grouping of units is done on covariates after getting the observational data. There covariate adjustment is done to reduce the confounding bias. For instance, \citet{rosenbaum1983central} provided a way to form blocks by matching the observation on the propensity score, which is famously termed as \textit{propensity score matching} (PSM). General concerns with matching have been raised by \citet{pearl2009causality}, who has argued that hidden bias may actually increase because matching on observed variables may unleash bias due to dormant unobserved confounders. Similarly, \citet{pearl2009causality} has argued that bias reduction can only be assured (asymptotically) by modeling the qualitative causal relationships between treatment, outcome, observed, and unobserved covariates. Confounding occurs when the experimenter is unable to control for alternative, non-causal explanations for an observed relationship between independent and dependent variables. Such control should satisfy the \textit{back-door criterion} \citet{pearl2009causality}.

\subsection{Challenges with Blocking} \label{sec:challenges}
We observed that in experimental studies under non-homogeneity of the experimental units, blocking improves the precision of causal effect estimation. However, the practical difficulty with blocking is that depending on the number of covariates and the number of distinct values (denoted as $v(\cdot)$) of each covariate, the number of blocks can be very large. For covariates in the set $\mathcal{Z}$, we need to form $\prod_{Z \in \mathcal{Z}}v(Z)$ different blocks. For example, if we want to study the effect of a drug on curing some heart disease where the subjects under consideration have the following attributes (which can potentially affect the effectiveness of the drug). Gender: Male and Female, i.e., $v(\text{Gender})=2$, Age: $<$25, 25-45, 45-65, $>$65, i.e., $v(\text{Age})=4$, Weight: Underweight, Normal, Overweight, Obese I, Obese II, i.e., $v(\text{Weight})=5$, Blood Pressure: Normal, Prehypertension, Hypertension I, Hypertension II, Hypertensive Crisis, i.e., $v(\text{Blood Pressure})=5$, and Bad Cholesterol: Optimal, Above Optimal, Borderline High, High, Very High, i.e., $v(\text{Bad Cholesterol})=5$. Thus, we need to form $2\times4\times5\times5\times5=1000$ blocks. Performing a randomized experiment with a large number of blocks can be very costly. Sometimes, it may not be feasible as the number of blocks can be larger than the number of subjects. This would cause some of the blocks to be empty. For instance, there may not be any male subjects under the age of 25 who are Obese II with a Hypertensive Crisis and Optimal Cholesterol level. 

%For further discussion on the challenges and importance of blocking refer to \cite{higgins2016improving} and \citet{burger2020importance}, respectively. 
Other than the economic aspects and some blocks being empty, there are reasons why some variables should never be used for forming blocks. Refer to \cref{sec:stable_blocking} for details.

% \begin{enumerate}
% \item Gender: Male and Female, i.e., $v(\text{Gender})=2$,
% \item Age: $<$25, 25-45, 45-65, $>$65, i.e., $v(\text{Age})=4$,
% \item Weight: Underweight, Normal, Overweight, Obese I, Obese II, i.e., $v(\text{Weight})=5$,
% \item Blood Pressure: Normal, Prehypertension, Hypertension I, Hypertension II, Hypertensive Crisis, i.e., $v(\text{Blood Pressure})=5$, and
% \item Bad Cholesterol: Optimal, Above Optimal, Borderline High, High, Very High, i.e., $v(\text{Bad Cholesterol})=5$.
% \end{enumerate}

%Furthermore, the cost of forming blocks may differ across covariates. Therefore, some covariates may be statistically very relevant but still economically very expensive. 

\subsection{Problem Statement}
So far, we observed that blocking improves the precision of causal effect estimation. However, in situations when the number of blocks to be formed is very large, blocking becomes costly and/or infeasible. One possible way to reduce the number of blocks is to form blocks using some but not all covariates. But the question is which covariates should be preferred over others while forming blocks? One possible way is to select the (smallest) set of covariates that leads to maximum precision in causal effect estimation. In the context of estimating the effect of treatment in the population, $\beta$, (discussed in \cref{sec:gain_in_precision}), it means finding the smallest set, $\mathcal{Z}$, that minimizes $\Var(\hat{\beta}_\mathcal{Z})$.

We next formalize the problem of interest in this paper as follows. We are given a directed acyclic causal graph, $\mathcal{G}$, that depicts the causal relationships among some observed variables, $\mathcal{V}$, and unobserved variables, $\mathcal{U}$. We are interested in studying the causal effect of $X\in\mathcal{V}$ (treatment) on $Y\in\mathcal{V}$ (response) by performing a randomized block experiment. The set of observed covariates is $\mathcal{C}:=\mathcal{V} \backslash \{X,Y\}$. 

Studying the causal effect of $X$ on $Y$ means learning the (interventional) probability distribution, $\mathbb{P}(Y|do(X))$. We can write $\mathbb{P}(Y=y|do(X=x))$ as
\begin{align}
    \mathbb{P}(Y=y|do(X=x)) = \frac{\P(Y=y \cap do(X=x))}{\P(do(X=x))}
\end{align}
For estimating the above probability, we perform an RBD by forming blocks using covariates in $\mathcal{Z} \subseteq \mathcal{V} \backslash \{X,Y\}$, and similar to the estimation of $\E(Y|do(X))$, we define an estimate of $\mathbb{P}(Y=y|do(X=x))$ as
\begin{align}
    \hat{\P}_\mathcal{Z}&(Y=y|do(X=x)) := \sum_{\mathcal{Z} = z}\frac{\hat{\P}(Y=y \cap do(X=x) \cap \mathcal{Z} = z)}{\hat{\P}(do(X=x) \cap \mathcal{Z} = z))} \hat{\P}(\mathcal{Z}=z)
\end{align}
where $\hat{\P}(\cdot)$ are the sample relative frequencies.

It is desirable to select the $\mathcal{Z}$ such that $\Var(\hat{\P}_\mathcal{Z}(Y=y|do(X=x)))$ is minimized, i.e., maximum gain in precision. For ease of notation, we define $\Var(\hat{\P}_\mathcal{Z}(Y|do(X))):= \Var(\hat{\P}_\mathcal{Z}(Y=y|do(X=x)))$.

\begin{problem} \label{problem:optimal_blocking}  
Given a directed acyclic graph, $\mathcal{G}$, that depicts the causal relationships among some observed variables, $\mathcal{V}$, and unobserved variables, $\mathcal{U}$; treatment, $X\in\mathcal{V}$, and response, $Y\in\mathcal{V}$, obtain a smallest subset, $\mathcal{Z}^*$, of the set of observed covariates, $\mathcal{C}:=\mathcal{V} \backslash \{X,Y\}$, such that
\begin{align}
    \mathcal{Z}^* \in \argmin_{\mathcal{Z}}\Var(\hat{\P}_\mathcal{Z}(Y|do(X))).
\end{align}
\end{problem}

\begin{note}
\textup{
It is reasonable to assume that using some expert knowledge, we have access to the underlying causal graph $\mathcal{G}$ and do not know the strengths/weights of the causal connections depicted in this graph \citep{kyriacou2022using}. For instance, experts may tell us that alcohol consumption causes high blood pressure but may not have the knowledge of the magnitude of this causation. We can also construct the underlying causal graph using some observational data if it is available \citep{nordon2019building}.
}
\end{note}

\begin{note}
\textup{
While performing blocking for the minimization of the variance of the estimate of the causal effect, it is important to ensure that we are still able to accurately estimate the causal effect of interest. As introduced in \cref{sec:motivation}, we want the chosen set of covariates to be \textit{stable}, i.e. we exclude the covariates that one should never be used to create blocks. We formally motivate and define the notion of stability of the solution to \cref{problem:optimal_blocking} in \cref{sec:stable_blocking}. We also provide a method of achieving stability, i.e. finding and excluding the covariates that lead to inaccurate causal effect estimation. 
}
\end{note} 

\begin{note}
\textup{In experimental design, the term `block' refers to a subset of the experimental units that are homogenous with respect to some covariates while in causal graphical models, it refers to an obstruction in some causal path. For instance, for an experiment, a group of smokers can be a block while in causal graphical models, a common cause (confounder) blocks/obstructs a causal path.}
\end{note}

%\textbf{Note.} If we use the set of all observed covariates, $\mathcal{C}$, for forming the blocks then it would lead to a minimum variance but it is not necessarily the smallest set. In fact, $\mathcal{C}$ is the largest such set. The question of interest is, can we prune $\mathcal{C}$ such that we do not lose anything in terms of the minimum variance but end up with a set that is a smaller set than $\mathcal{C}$?

% \begin{align*}
%     \Var(\hat{\P}_\mathcal{Z^*}(Y|do(X))) &\le \Var(\hat{\P}_\mathcal{Z}(Y|do(X))), \\ \forall \mathcal{Z} &\subseteq \mathcal{V} \backslash \{X,Y\}.
% \end{align*}
% %\textbf{Inputs:} $\mathcal{G}$, $X$, and $Y$.\\
% %\textbf{Output:} $\mathcal{Z}^*$

%\textit{What is the smallest subset of the set of observed covariates (excluding some forbidden variables if there are any) which will account (through blocking) for `maximum possible' elimination of variability in the response, and Therefore in the estimation of the causal effects, based on the causal structure (diagram) of the all the variables viz., treatment, response and covariates (observed and unobserved)?}

%The phrase \textit{maximum possible} in the above question emphasizes that there is always some uncontrollable variability in the response due to two reasons, viz., its own exogenous variable, and some unobserved (latent) confounders. Therefore hereafter the phrase \textit{controlling the variability in response} will always mean \textit{controlling the variability in response due to the observed variables only} unless specified otherwise.

%{\bf Need some text }

%\begin{definition}
%Any smallest subset of the set of observed covariates (excluding some forbidden variables if there are any) which will account (through blocking) for the maximum possible elimination of variability in the response is called a \textit{statistically optimal blocking set}.
%\end{definition} 
